A framework for coupled deformation-diffusion analysis with application to degradation/healing

This paper deals with the formulation and numerical implementation of a fully coupled continuum model for deformation-diffusion in linearized elastic solids. The mathematical model takes into account the effect of the deformation on the diffusion process, and the affect of the transport of an inert chemical species on the deformation of the solid. We then present a robust computational framework for solving the proposed mathematical model, which consists of coupled non-linear partial differential equations. It should be noted that many popular numerical formulations may produce unphysical negative values for the concentration, particularly, when the diffusion process is anisotropic. The violation of the non-negative constraint by these numerical formulations is not mere numerical noise. In the proposed computational framework we employ a novel numerical formulation that will ensure that the concentration of the diffusant be always non-negative, which is one of the main contributions of this paper. Representative numerical examples are presented to show the robustness, convergence, and performance of the proposed computational framework. Another contribution of this paper is to systematically study the affect of transport of the diffusant on the deformation of the solid and vice-versa, and their implication in modeling degradation/healing of materials. We show that the coupled response is both qualitatively and quantitatively different from the uncoupled response.

==> Sections/Coupled_Figures.tex <==
%------------------------------------------------------;
%  Figure: Abaqus result for square plate with a hole  ;
%------------------------------------------------------;
\begin{figure}
  \subfigure{\includegraphics[scale=0.35]
    {Figures/Abaqus/Abaqus_DMP_Square_Hole_Mesh.eps}}
  \subfigure{\includegraphics[scale=0.35]
    {Figures/Abaqus/Abaqus_DMP_Square_Hole_k1_10000_k2_1.eps}}
  \caption{ABAQUS simulation for plate with a square hole: 
    The left figure shows three-node triangular mesh used 
    in the simulation using Abaqus \cite{Abaqus_6.8-3}. The right 
    figure shows contours of concentration obtained using Abaqus 
    for the problem described in subsection \ref{SubSec:Plate_hole}.
    The white area in the right figure indicates the region in 
    which concentration has a \emph{negative} value. 
    Approximately 37 \% of nodes have negative values. The minimum 
    concentration obtained is $-0.0832$ (which is -4.16 \% off the 
    range of possible values: 0 to 2). We have taken $d_1 = 10000$, 
    $d_2 = 1$, and $\theta = -\pi / 6$. 
  \label{Fig:Coupled_Abaqus_DMP_plate_with_square_hole}}
\end{figure}

%------------------------------------------------------;
%  Figure: Pictorial description of convergence study  ;
%------------------------------------------------------;
 \begin{figure}
   \centering
   \psfrag{O}{O}
   \psfrag{b1}{specific body force is}
   \psfrag{b2}{given by equation \eqref{Eqn:Coupled_body_force_convergence}}
   \psfrag{f1}{volumetric source is}
   \psfrag{f2}{given by equation \eqref{Eqn:Coupled_volumetric_source_convergence}}
   \psfrag{up}{$\mathbf{u}(\mathbf{x}) = \mathbf{u}^{\mathrm{p}}(\mathbf{x})$}
   \psfrag{cp}{$c^{\mathrm{p}}(\mathbf{x}) = 1$}
   \psfrag{hp}{$h^{\mathrm{p}}(\mathbf{x}) = 0$}
   %
   \subfigure{\includegraphics[scale=0.7]
     {Figures/Numerical_convergence/Convergence_diffusion.eps}}
   \hspace{0.2in}
   %
   \subfigure{\includegraphics[scale=0.7]
     {Figures/Numerical_convergence/Convergence_deform.eps}}
   \caption{Numerical $h$-convergence: A pictorial description of 
     the boundary value problem. The computational domain is a bi-unit 
     square with origin denoted as O. The boundary conditions and the 
     volumetric source for the diffusion problem is shown in the 
     left figure. The (Dirichlet) boundary conditions and the 
     specific body force for the deformation problem is shown 
     in the right figure. The Dirichlet boundary conditions 
     $\mathbf{u}^{\mathrm{p}}(\mathbf{x})$ are prescribed by 
     directly evaluating the expressions for the displacement 
     given in equation \eqref{Eqn:displacement_convergence_study}. 
     \label{Fig:Coupled_convergence_pictorial}}
\end{figure}

%---------------------------------------------------------------;
%  Figure: Mesh for convergence study using T3 and Q4 elements  ;
%---------------------------------------------------------------;
\begin{figure}
  \subfigure{\includegraphics[scale=0.35]
    {Figures/Numerical_convergence/Mesh_21_T3/Convergence_mesh_T3.eps}
    \label{Fig:Coupled_convergence_T3_mesh}}
    %
  \subfigure{\includegraphics[scale=0.35]
    {Figures/Numerical_convergence/Mesh_21_Q4/Convergence_mesh_Q4.eps}}
    %
  \caption{Numerical $h$-convergence: This figure shows 
    the typical three-node triangular and four-node 
    quadrilateral meshes used in the numerical convergence 
    analysis. Both these meshes have 21 nodes along each 
    side. For the numerical convergence analysis, these 
    meshes are subdivided in a hierarchical manner to 
    obtain a series of meshes. 
    \label{Fig:Coupled_convergence_mesh}}
\end{figure}

%------------------------------------------------------------------------;
%  Figure: Concentration profile for convergence study using T3 element  ;
%------------------------------------------------------------------------;
\begin{figure}
  \subfigure{\includegraphics[scale=0.35]
    {Figures/Numerical_convergence/Mesh_21_T3/Diffusion_AS_T3.eps}}
    %
  \subfigure{\includegraphics[scale=0.35]
    {Figures/Numerical_convergence/Mesh_21_T3/Diffusion_Convergence_T3.eps}}
    %
  \caption{Numerical $h$-convergence: Comparison of concentration
    profile from analytical solution (left) to that of the numerical
    study (right) using three-node triangular mesh shown in Figure 
    \ref{Fig:Coupled_convergence_mesh}.
    \label{Fig:Coupled_convergence_conc_comparison}}
\end{figure}

\clearpage
\newpage

%--------------------------------------------------------------;
%  Figure: Concentration convergence using T3 and Q4 elements  ;
%--------------------------------------------------------------;
\begin{figure}
  \subfigure{\includegraphics[scale=0.22]{Figures/Numerical_convergence/Convergence_conc_T3.eps}}
  % 
  \subfigure{\includegraphics[scale=0.22]{Figures/Numerical_convergence/Convergence_conc_Q4.eps}}
  % 
  \caption{Numerical $h$-convergence: Convergence of the proposed 
    computational framework with respect to the \emph{concentration 
      field} is illustrated in this figure. We show the convergence 
    in $L^2$-norm and $H^1$-seminorm for three-node triangular (left) 
    and four-node quadrilateral (right) finite elements. 
    \label{Fig:Coupled_convergence_conc}}
\end{figure}

%-------------------------------------------------------------;
%  Figure: Displacement convergence using T3 and Q4 elements  ;
%-------------------------------------------------------------;
\begin{figure}
  \subfigure{\includegraphics[scale=0.22]{Figures/Numerical_convergence/Convergence_disp_T3.eps}}
  % 
  \subfigure{\includegraphics[scale=0.22]{Figures/Numerical_convergence/Convergence_disp_Q4.eps}}
  % 
  \caption{Numerical $h$-convergence: Convergence of the proposed 
    computational framework with respect to the \emph{displacement 
    field} is illustrated in this figure. We show the convergence 
    in $L^2$-norm and $H^1$-seminorm for three-node triangular 
    (left) and four-node quadrilateral (right) finite elements. 
    \label{Fig:Coupled_convergence_disp}}
\end{figure}

%--------------------------------------------------------------------;
%  Figure: Pictorial description of cantilever beam with edge shear  ;
%--------------------------------------------------------------------;
 \begin{figure}
   \centering
   \psfrag{a1}{1.0}
   \psfrag{c1}{\rotatebox{90}{0.1}}
   \psfrag{b1}{$\mathbf{b}(\mathbf{x}) = \mathbf{0}$}
   \psfrag{d1}{uniformly distributed shear = 500}
   \psfrag{a11}{$c^{\mathrm{p}}(\mathbf{x}) = 0$}
   \psfrag{d11}{$c^{\mathrm{p}}(\mathbf{x}) = 0$}
   \psfrag{c11}{\rotatebox{90}{$h^{\mathrm{p}}(\mathbf{x}) = 0$}}
   \psfrag{e11}{\rotatebox{-90}{$h^{\mathrm{p}}(\mathbf{x}) = 0$}}
   \psfrag{b11}{$f(\mathbf{x}) = 10^4$}
   \psfrag{O}{O}
   %
   \includegraphics[scale=1.0]{Figures/Cantilever_Beam/CB_deform_diffusion.eps}
   %
   \caption{Cantilever beam with edge shear: A pictorial description of 
     the boundary value problem with origin at `O'. The boundary conditions 
     and the specific body force for the deformation problem is shown 
     in the top figure and the boundary conditions and the 
     volumetric source for the diffusion problem is shown in the 
     bottom figure. 
     \label{Fig:Coupled_CB_edgeshear}}
\end{figure}

%-----------------------------------------------------------;
%  Figure: Concentration cantilever beam due to edge shear  ; 
%-----------------------------------------------------------;
\begin{figure}
	\centering
	\includegraphics[scale=0.75]{Figures/Cantilever_Beam/CBES/Diffusion_CBES.eps}
	\caption{Cantilever beam with edge shear: Four-node quadrilateral mesh 
	  (top figure) used in the numerical study and comparison of the 
	  concentration profiles (in the order of precedence) for three
	  different values of $\Phi_S$ being equal to $5, \; 10 \; 
	  \mathrm{and} \; 20$}.
	\label{Fig:Diffusion_CB_Edgeshear}
\end{figure}

%---------------------------------------------------------------------------;
%  Figure: Pictorial description of simply supported beam with self weight  ;
%---------------------------------------------------------------------------;
 \begin{figure}
   \centering
   \psfrag{a1}{1.0}
   \psfrag{c1}{\rotatebox{90}{0.1}}
   \psfrag{b1}{$\mathbf{b}(\mathbf{x}) = -10 \, \hat{\mathbf{e}}_y$}
   \psfrag{a11}{$c^{\mathrm{p}}(\mathbf{x}) = 0$}
   \psfrag{d11}{$c^{\mathrm{p}}(\mathbf{x}) = 0$}
   \psfrag{c11}{\rotatebox{90}{$h^{\mathrm{p}}(\mathbf{x}) = 0$}}
   \psfrag{e11}{\rotatebox{-90}{$h^{\mathrm{p}}(\mathbf{x}) = 0$}}
   \psfrag{b11}{$f(\mathbf{x}) = 10^3$}
   \psfrag{O}{O}
   %
   \includegraphics[scale=1.0]{Figures/Simply_supported_beam/SS_deform_diffusion.eps}
   %
   \caption{Simply supported beam under self-weight:
     A pictorial description of the boundary value problem with 
     origin at `O'. The boundary conditions and the specific body 
     force for the deformation problem is shown in the top figure 
     and the boundary conditions and the volumetric source for the
     diffusion problem is shown in the bottom figure. 
     \label{Fig:Coupled_SS_selfweight}}
\end{figure}

%---------------------------------------------------;
%  Figure: Simply supported beam under self-weight  ; 
%---------------------------------------------------;
\begin{figure}
	\centering
	\includegraphics[scale=0.75]{Figures/Simply_supported_beam/Diffusion_SSUDL.eps}
	\caption{Simply supported beam under self-weight: Four-node quadrilateral mesh 
	  (top figure) used in the numerical study and comparison of the 
	  concentration profiles (in the order of precedence) for three
	  different values of $\eta_S$ being equal to $1, \; 10^3 \; 
	  \mathrm{and} \; 2 \times 10^4$}.
	\label{Fig:Diffusion_SS_selfweight}
\end{figure}

%----------------------------------------------------------------;
%  Figure: Pictorial description of fixed beam with self weight  ;
%----------------------------------------------------------------;
 \begin{figure}
   \centering
   \psfrag{a1}{1.0}
   \psfrag{c1}{\rotatebox{90}{0.1}}
   \psfrag{b1}{$\mathbf{b}(\mathbf{x}) = -10 \, \hat{\mathbf{e}}_y$}
   \psfrag{a11}{$c^{\mathrm{p}}(\mathbf{x}) = 0$}
   \psfrag{d11}{$c^{\mathrm{p}}(\mathbf{x}) = 0$}
   \psfrag{c11}{\rotatebox{90}{$h^{\mathrm{p}}(\mathbf{x}) = 0$}}
   \psfrag{e11}{\rotatebox{-90}{$h^{\mathrm{p}}(\mathbf{x}) = 0$}}
   \psfrag{b11}{$f(\mathbf{x}) = 10^2$}
   \psfrag{O}{O}
   %
   \includegraphics[scale=1.0]{Figures/Fixed_beam/FB_deform_diffusion.eps}
   %
   \caption{Fixed beam under self-weight:
     A pictorial description of the boundary value problem with 
     origin at `O'. The boundary conditions and the specific body 
     force for the deformation problem is shown in the top figure 
     and the boundary conditions and the volumetric source for the
     diffusion problem is shown in the bottom figure. 
     \label{Fig:Coupled_FB_selfweight}}
\end{figure}

%-----------------------------------------------------;
%  Figure: Concentration fixed beam with self-weight  ;
%  (Tension, compression and shear)                   ;
%-----------------------------------------------------;
\begin{figure}
	\centering
	\includegraphics[scale=0.75]{Figures/Fixed_beam/Diffusion_FBUDL.eps}
	\caption{Fixed beam under self-weight: Four-node quadrilateral mesh 
	  (top figure) used in the numerical study and comparison of the 
	  concentration profiles (in the order of precedence) for three
	  different values of $\Phi_T$ being equal to $1, \; 5 \; 
	  \mathrm{and} \; 7$.
	\label{Fig:Diffusion_FB_selfweight_mudunuru}}
\end{figure}

%-----------------------------------------------------;
%  Figure: Concentration fixed beam with self-weight  ;
%  (Using Norm of epsilon)                            ; 
%-----------------------------------------------------;
\begin{figure}
	\centering
	\includegraphics[scale=0.75]{Figures/Fixed_beam/Diffusion_FBUDL_norm.eps}
	\caption{Fixed beam under self-weight: The concentration profiles obtained using
	  the diffusivity model \eqref{Eqn:Coupled_diffusivity_norm} as outlined in 
	  Reference \cite{Karra_Rajagopal_degradation_arXiv_2010}. 
	\label{Fig:Diffusion_FB_selfweight_karra}}
\end{figure}

%------------------------------------------------------;
%  Figure: Pictorial description of plate with a hole  ;
%------------------------------------------------------;
 \begin{figure}
   \centering
   \psfrag{a1}{\rotatebox{90}{1.0}}
   \psfrag{b1}{1.0}
   \psfrag{c1}{\rotatebox{90}{$1/9$}}
   \psfrag{d1}{$1/9$}
   \psfrag{O}{O}
   \psfrag{H}{H}
   \psfrag{e1}{$c^{\mathrm{p}}(\mathbf{x}) = 1$}
   \psfrag{f1}{$c^{\mathrm{p}}(\mathbf{x}) = 0$}
   %
   \subfigure{\includegraphics[scale=0.95]
     {Figures/Plate_with_hole/Plate_with_hole_New.eps}}
   %
   \hspace{0.5in}
   %
   \subfigure{\includegraphics[scale=0.31]
     {Figures/Plate_with_hole/Diffusion_POH_mesh.eps}} 
   %
   \caption{Plate with a hole under self-weight:
     A pictorial description of the dimensions for a plate with 
     a hole in the left figure and three-node triangular unstructured 
     mesh used in our numerical study in right figure. The origin is 
     located at `O' and the vertex `H' of the hole at $\left(
     \frac{4}{9}, \, \frac{4}{9}\right)$. Displacements at 
     the boundary of the hole and traction at the boundary of 
     the plate are zero. In the region between the plate and 
     the hole,  the body force is $\mathbf{b}(\mathbf{x}) = 
     -10 \, \hat{\mathbf{e}}_y$ and the volumetric source is 
     $f(\mathbf{x}) = 0$. The concentration at the boundary 
     of the hole is $1$ and at the boundary of the plate 
     is $0$. 
     \label{Fig:Plate_with_hole_pictorial}}
\end{figure}

%-------------------------------------------------------;
%  Figure: Concentration profile for plate with a hole  ;
%-------------------------------------------------------;
\begin{figure}
  \subfigure{\includegraphics[scale=0.35]
    {Figures/Plate_with_hole/Galerkin/Diffusion_POHSG.eps}
    \label{Fig:Plate_with_hole_concentration_Galerkin}}
    %
  \subfigure{\includegraphics[scale=0.35]
    {Figures/Plate_with_hole/Non_Negative/Diffusion_POHNN.eps}}
    %
  \caption{Plate with a hole under self-weight: This figure 
    compares concentration profiles from the standard Galerkin 
    formulation (left figure) and the non-negative formulation 
    (right figure). The white area in the left figure indicates 
    the regions in which concentration is negative. The violations 
    also include that are of order machine precision. 
    \label{Fig:Plate_with_hole_concentration}}
\end{figure}

%-----------------------------------------------------;
%  Figure: Degradation profile for plate with a hole  ;
%-----------------------------------------------------;
\begin{figure}
  \subfigure{\includegraphics[scale=0.35]
    {Figures/Plate_with_hole/Galerkin/Heal_Degrade_POHSG.eps}}
    %
  \subfigure{\includegraphics[scale=0.35]
    {Figures/Plate_with_hole/Non_Negative/Heal_Degrade_POHNN.eps}}
    %
  \caption{Plate with a hole under self-weight: This figure compares 
    degradation profiles from the standard Galerkin formulation 
    (left figure) and the non-negative formulation (right figure). 
    The red area indicates the regions in which the material is 
    degrading and the green area indicates the regions in which 
    the material is healing (which is because unphysical negative 
    value for the concentration). In this figure we do not consider 
    negative values of order machine precision as violations. 
    \label{Fig:Plate_with_hole_degradation}}
\end{figure}

%------------------------------------------------------------;
%  Figure: Pictorial description of a beam with three holes  ;
%------------------------------------------------------------;
 \begin{figure}
   \centering
   \psfrag{a1}{\rotatebox{90}{$1.0$}}
   \psfrag{b1}{$10.0$}
   \psfrag{O}{O}
   \psfrag{A}{A}
   \psfrag{B}{B}
   \psfrag{C}{C}
   \psfrag{H1}{$\mathrm{H}_1$}
   \psfrag{H2}{$\mathrm{H}_2$}
   \psfrag{H3}{$\mathrm{H}_3$}
   %
   %\includegraphics[scale=1.1]
   \includegraphics[height = 0.14\textheight, width = 0.88\textwidth]
     {Figures/Beam_with_three_holes/Beam_with_three_holes_New.eps}
   %
   \caption{Beam with three holes under self-weight:
     A pictorial description of the dimensions for a beam with 
     three square holes. The dimensions of each hole are 
     $0.4 \times 0.4$. The origin is located at `O' and the vertices 
     `$\mathrm{H}_1$', `$\mathrm{H}_2$' and `$\mathrm{H}_3$' of 
     the holes `A, B, C' are at $\left(1.8, \, 0.3\right)$, $\left(4.8, \, 
     0.3\right)$ and $\left(7.8, \, 0.3\right)$. Displacements at 
     the boundary of the holes and traction at the boundary of the 
     beam are zero. In the region between the beam and the holes, 
     the body force is $\mathbf{b}(\mathbf{x}) = -10 \, 
     \hat{\mathbf{e}}_y$ and the volumetric source is 
     $f(\mathbf{x}) = 0$. The concentration at the boundary 
     of the holes is $1$ and at the boundary of the beam is $0$. 
     \label{Fig:Beam_with_three_holes_pictorial}}
\end{figure}

%-------------------------------------------------------------;
%  Figure: Concentration profile for a beam with three holes  ;
%-------------------------------------------------------------;
\begin{figure}
  \includegraphics[scale=0.75]
    {Figures/Beam_with_three_holes/Diffusion_B3H.eps}
    %
  \caption{Beam with three holes under self-weight: Comparison 
    of concentration profile from standard Galerkin formulation 
    (middle figure) to that of the non-negative formulation 
    (bottom figure). Three-node triangular unstructured mesh used 
    in the numerical study is shown in the top figure. The white 
    area in the middle figure indicates the region in which 
    concentration has a negative value. In this figure, the 
    white area also includes the regions with concentration 
    of order machine precision.
    \label{Fig:Beam_with_three_holes_concentration}}
\end{figure}

%---------------------------------------------------------;
%  Figure: Degradation profile for beam with three holes  ;
%---------------------------------------------------------;
\begin{figure}
  \includegraphics[scale=0.75]
    {Figures/Beam_with_three_holes/Heal_Degrade_B3H.eps}
    %
  \caption{Beam with three holes under self-weight: Comparison of 
    degradation profile from standard Galerkin formulation 
    (top figure) to that of the non-negative formulation 
    (bottom figure). The red area indicates material is degrading
    and the green area indicates the material is healing (because 
    of unphysical negative value for the concentration). In this 
    figure we do not consider the negative values that are of 
    order machine precision as violations. 
    \label{Fig:Beam_with_three_holes_degradation}}
\end{figure}

\clearpage

%------------------------------------------------------;
%  Figure: Staggered scheme plots for                  ;
%          cantilever,simply supported and fixed beams ;
%          plate with a hole and beam with three holes ;
%------------------------------------------------------;
\begin{figure}
  \subfigure{\includegraphics[scale=0.35]
    {Figures/Staggered_ActiveSet_Plots/Stagg_ActSet_CSSF_Beams.eps}}
  %
  \vspace{0.1in}  
  % 
  \subfigure{\includegraphics[scale=0.35]
    {Figures/Staggered_ActiveSet_Plots/Stagg_ActSet_Domain_Holes.eps}
    \label{Fig:Coupled_staggered_conc_domain_holes}}
  % 
  \caption{Convergence of staggered coupling algorithm: We have plotted 
    $\mathrm{ln}[\| \boldsymbol{c}^{(i)} - \boldsymbol{c}^{(i - 1)}\| ]$ 
    with respect to iteration number for various problems. The stopping 
    criterion in the staggered coupling algorithm is $\|\boldsymbol{c}^{(i)} 
    - \boldsymbol{c}^{(i-1)}\| < \epsilon^{(c)}_{\mathrm{TOL}}$. As one can 
    see from the figure, the staggered coupling algorithm converges 
    for all the chosen problems. Also, note that the algorithm need 
    not converge monotonically, which is evident in the case of 
    plate with a hole test problem. 
    \label{Fig:Coupled_staggered_conc}}
\end{figure} 

%------------------------------------------------------;
%  Figure: Active set strategy plots for               ;
%          cantilever,simply supported and fixed beams ;
%          plate with a hole and beam with three holes ;
%------------------------------------------------------;
\begin{figure}
  \subfigure{\includegraphics[scale=0.35]
    {Figures/Staggered_ActiveSet_Plots/ActSet_CSSF_Beams.eps}}
  %
  \vspace{0.1in}  
  % 
  \subfigure{\includegraphics[scale=0.35]
    {Figures/Staggered_ActiveSet_Plots/ActSet_Domain_Holes.eps}}
  % 
  \caption{Convergence of the active-set strategy: This figure shows 
    the number of iterations taken by the active-set strategy for each 
    iteration in the staggered coupling algorithm for various test 
    problems. \label{Fig:Coupled_active_set_conc}}
\end{figure}
 


==> Sections/S1_Coupled_Introduction.tex <==
%****************************************;
%                                        ;
%  NAME                                  ;
%    S1_Coupled_Introduction.tex         ;
%                                        ;
%****************************************;
\section{INTRODUCTION}
\label{Sec:Coupled_Introduction}
In this paper we present a continuum mathematical model and 
a computational framework for degradation/healing in elastic 
solids due to the presence of a solute. We shall neglect chemical 
reactions as well as thermal effects. We shall also assume that the 
strains in the solid are small. The deformation is coupled with the 
diffusion process, and the diffusion process is in turn coupled with 
the deformation of the solid. The chosen problem belongs to a 
broader class of problems, namely, coupled deformation-diffusion 
problems. 

Coupled deformation-diffusion problems arise in many civil 
engineering, material science, and polymer science applications. 
An important example is degradation/healing of materials and 
structures. Many man-made and natural materials degrade/heal 
due to environmental conditions, and  structural components and 
superstructures are constantly exposed to adverse conditions. The 
fate of the transport of a diffusant will in turn depend on the 
deformation of the solid.
%
Some other examples of coupled deformation-diffusion problems 
are moisture damage in cementitious materials 
\cite{2004_Kuhl_Bangert_Meschke_IJSS_v41_p15,
  2004_Kuhl_Bangert_Meschke_IJSS_v41_p41} and asphalt 
\cite{2003_Cheng_Little_Lytton_Holste_v1832_p42,
  2004_Kim_Little_Lytton_v1891_p48}, hydrogen 
embrittlement \cite{Sofronis_JMPS_1995_v43_p1385,
  Woodtli_Kieselbach_EFA_2000_v7_p427}, curing of ceramics 
\cite{Marras_Ihtiaris_Hatzitrifon_Sikalidis_Aifantis_JECS_2000_v20_p243}, 
and swelling of polymers and composites \cite{Wu_Peppas_JAPS_1993_v49_p1845,
  1987_Weitsman_IJSS_v23_p1003}. 

The governing equations of a deformation-diffusion problem are 
coupled non-linear partial differential equations. That is, the 
mechanical variables (strains and stresses) and diffusive variables 
(concentration and mass flux) are coupled through constitutive 
relations. It is (in general) not possible to obtain analytical 
solutions for these kinds of problems, and one has to resort to 
numerical techniques to solve practical problems. Despite the 
importance of coupled deformation-diffusion problems, there is 
no \emph{robust} and \emph{reliable} computational framework 
for solving such coupled problems. In particular, the existing 
numerical studies have one or more of the following limitations: 
\begin{itemize}
\item considered academic and unrealistic problems like infinite 
  slabs and infinite cylinders,  
\item did not consider anisotropic diffusion and/or 
  assumed the medium to be homogeneous, or 
\item did not consider the fact that conventional numerical 
  formulations and finite element packages produce unphysical 
  negative values for the concentration in solving diffusion-type 
  equations. 
\end{itemize}

%===================================================================;
%  Subsection: Non-negative solutions for diffusion-type equations  ;
%===================================================================;
\subsection{Maximum principles and non-negative solutions for diffusion-type equations}
Predictive numerical simulations require accurate and reliable discretization 
methods. The resulting discrete systems must inherit or mimic fundamental 
properties of continuous systems. Maximum principles form an important set 
of properties for diffusion-type equations as these maximum principles have 
mathematical implications and physical consequences. In the study on partial 
differential equations, maximum principles are often used in existence theorems, 
and in obtaining point-wise estimates. For further details on (continuous) maximum 
principles refer to \cite{McOwen,Evans_PDE,Gilbarg_Trudinger,Fraenkel_maximum_principles,
Protter_Weinberger,Han_Lin}. 

A direct consequence of maximum principles for diffusion-type is the non-negativity 
of the solution (under appropriate conditions on the source and boundary conditions). 
Physical quantities like concentration of a diffusant should be non-negative by their 
nature and their approximations should also be non-negative as well. The question 
to ask is whether a chosen numerical formulation satisfies these maximum principles 
and meet the non-negative constraint. The discrete version of maximum principles 
is commonly referred as \emph{discrete maximum principles}.  

Many existing numerical formulations and packages do not satisfy the maximum principles. 
They may produce negative values for the primary variables in diffusion-type equations (that is, 
negative values for the concentration and temperature). \emph{It should be emphasized that the 
violation is not mere numerical noise, that is, the violations will be much larger than the machine 
precision and cannot be neglected.}

For example, in Figure \ref{Fig:Coupled_Abaqus_DMP_plate_with_square_hole}, 
we have shown that the contours of concentration obtained using Abaqus 
\cite{Abaqus_6.8-3} for pure diffusion. The uncoupled problem is similar to one 
considered in Section \ref{Sec:Coupled_Numerical_results}. As one can 
see from the figure, significant part of the domain has negative solution. 
The minimum value of the concentration is approximately $-0.0832$, which 
is $4.16 \%$ off the range of possible values (which is between 
$0$ and $2$). In a subsequent section we show that the classical single-field 
Galerkin formulation produces negative values for the concentration for the 
same test problem (see Figure \ref{Fig:Plate_with_hole_concentration}), and 
produces (qualitatively and quantitatively) wrong results for a coupled 
deformation-diffusion problem.  
%
Furthermore, Nakshatrala and Valocchi \cite{Nakshatrala_Valocchi_JCP_2009_v228_p6726} 
have shown that the lowest order Raviart-Thomas \cite{Raviart_Thomas_MAFEM_1977_p292} 
and variational multiscale \cite{Masud_Hughes_CMAME_2002_v191_p4341,
Nakshatrala_Turner_Hjelmstad_Masud_CMAME_2006_v195_p4036} mixed formulations 
violate discrete maximum principle and produce negative solutions for pure 
diffusion equation. Nagarajan and Nakshatrala \cite{Nagarajan_Nakshatrala_IJNMF_2010} 
have shown that the single-field formulation violates discrete maximum principles for 
diffusion with decay. 

%============================;
%  Subsection: Our approach  ;
%============================;
\subsection{Our approach}
Herein, we will consider realistic problems, allow the medium to be 
inhomogeneous, consider anisotropic diffusion, and develop a robust 
computational framework that will always produce physically meaningful 
non-negative values for the concentration of the diffusant on general 
computational grids. The computational framework will consist of a 
non-negative formulation for diffusion equation, a single-field 
formulation for the deformation problem, and a staggered coupling 
algorithm. 

We employ a staggered coupling technique (also known as partitioned 
solution approach) to couple individual analyses to obtain the coupled 
response. The non-negative formulation for diffusion is developed by 
extending the Galerkin formulation using convex programming, which 
produces (physical) non-negative solutions for the concentration 
even on general computational grids with low-order finite elements 
(linear three-node triangular, bilinear four-node quadrilateral, 
linear four-node tetrahedron, and tri-linear eight-node brick 
elements). The proposed non-negative formulation being applicable 
only to low-order finite elements is not a limitation as low-order 
finite elements remain quite popular in the solution of practical 
problems. (This is particularly true for large-scale simulations 
with complex geometries because of the inherent simplicity of 
low-order elements. Another reason is that adaptive mesh-generation 
techniques are simpler and tend to perform better with low-order 
finite elements.)

%================================================;
%  Subsection: Main contributions of this paper  ;
%================================================;
\subsection{Main contributions of this paper} 
Some of the main contributions of this paper are as follows: 
%
\begin{enumerate}[(1)]
\item We presented a mathematical model for diffusion of an inert chemical 
  species in an elastic deformable solid that takes into account the effect 
  of diffusant on the deformation. The model is \emph{truly coupled} in the 
  sense that the deformation of the solid will be affected by the diffusion 
  process, and the diffusion process is in turn affected by the deformation 
  of the solid. Such a coupled deformation-diffusion model is suitable to 
  study degradation/healing in elastic solids. We restricted our model to 
  steady-state. 
  % 
\item We presented a robust computational framework for performing 
  deformation--diffusion analysis. The framework includes a solver 
  for deformation, a non-negative solver for tensorial-diffusion, and 
  a coupling algorithm to couple the individual deformation and 
  diffusion analyses. The coupling algorithm is a staggered algorithm 
  in which deformation and diffusion sub-problems are solved in an 
  iterative fashion until convergence. \emph{An important aspect of 
  the proposed framework is that it employs a novel numerical formulation 
  that ensures non-negative solutions for the concentration of the diffusant}. 
  % 
\item Using the proposed computational framework, we solved some 
  realistic finite domain problems on general computational meshes. 
  Also, we systematically studied the effect of the concentration of the 
  diffusant on the deformation of the solid and vice-versa, and their 
  implications on degradation/healing of materials and structures.
\end{enumerate}

%==============================================================;
%  Subsection: An outline of this paper and symbolic notation  ;
%==============================================================;
\subsection{An outline of this paper and symbolic notation}
The remainder of this paper is organized as follows. Section 
\ref{Sec:Coupled_Mathematical_model} presents a mathematical model for 
degradation/healing of a deformable elastic solid. The mathematical model 
will require performing coupled deformation-diffusion analysis. In Section 
\ref{Sec:Coupled_Computational_framework} we present a fully coupled computational 
framework for deformation-diffusion analysis. The proposed computational framework 
will contain a non-negative formulation for tensorial-diffusion equation on general 
computational grids (which will always produce physically meaningful non--negative 
values for the concentration), a numerical solver for deformation, and a staggered 
coupling algorithm for coupling individual diffusion and deformation numerical 
solvers. In Section \ref{Sec:Coupled_Numerical_results}, representative numerical 
examples will be presented to illustrate the performance of the proposed coupled 
deformation-diffusion computational framework. Conclusions are drawn in Section 
\ref{Sec:Coupled_Conclusions}.

The symbolic notation adopted in this paper is as follows. We shall 
make a distinction between vectors in the continuum and finite element 
settings. Similarly, we make a distinction between second-order tensors 
in the continuum setting versus matrices in the context of the finite element 
method. The continuum vectors are denoted by lower case boldface normal letters, 
and the second-order tensors will be denoted using upper case boldface normal 
letters (for example, vector $\mathbf{u}$ and second-order tensor $\mathbf{T}$). 
In the finite element context, we shall denote the vectors using lower case 
boldface italic letters, and the matrices are denoted using upper case boldface 
italic letters (for example, vector $\boldsymbol{v}$ and matrix $\boldsymbol{K}$). 
Other notational conventions adopted in this paper are introduced as needed.

==> Sections/S2_Coupled_Mathematical_model.tex <==
%********************************************************************;
%                                                                    ;
%  Section: A mathematical model for coupled deformation-diffusion   ;
%                                                                    ;
%********************************************************************;
\section{A MATHEMATICAL MODEL FOR COUPLED DEFORMATION-DIFFUSION}
\label{Sec:Coupled_Mathematical_model}
%
Consider an \emph{inert} (chemical or biological) species being diffused through 
a deformable elastic solid. We now present a simple mathematical model for such 
a process. Let $\Omega \subset \mathbb{R}^{nd}$ be a bounded open domain, where 
``$nd$" denotes the number of spatial dimensions. The boundary $\partial \Omega$ 
is assumed to be piecewise smooth. Mathematically, $\partial \Omega = \bar{\Omega} 
- \Omega$, where $\bar{\Omega}$ is the set closure of $\Omega$. A spatial point in 
$\bar{\Omega}$ is denoted by $\mathbf{x}$. The gradient and divergence operators 
with respect to $\mathbf{x}$ are denoted by $\mathrm{grad}[\cdot]$ and $\mathrm{div}
[\cdot]$, respectively. The unit outward normal to the boundary is denoted by $\mathbf{n}
(\mathbf{x})$. We shall denote the displacement of the solid by $\mathbf{u}(\mathbf{x})$, 
and the concentration of the diffusant by $c(\mathbf{x})$. It is important to note that 
the concentration is a non-negative quantity, and a robust numerical solver should 
meet the non-negative constraint (which is not the case with many popular numerical 
schemes). 

For the deformation problem, the boundary is divided into two complementary 
parts: $\Gamma^{\mathrm{D}}_{u}$ on which the displacement vector is prescribed, 
and $\Gamma^{\mathrm{N}}_{u}$ on which the traction vector is prescribed. For 
the diffusion problem, the boundary is divided into $\Gamma^{\mathrm{D}}_{c}$ 
on which concentration is prescribed, and $\Gamma^{\mathrm{N}}_{c}$ on which 
the flux is prescribed. For well-posedness, we require that $\Gamma^{\mathrm{D}}_u 
\cap \Gamma^{\mathrm{N}}_u = \emptyset$, $\Gamma^{\mathrm{D}}_u \cup \Gamma^{\mathrm{N}}_u 
= \partial \Omega$, $\Gamma^{\mathrm{D}}_c \cap \Gamma^{\mathrm{N}}_c = \emptyset$, 
and $\Gamma^{\mathrm{D}}_c \cup \Gamma^{\mathrm{N}}_c = \partial \Omega$. In addition, 
we assume that $\mathrm{meas} (\Gamma^{\mathrm{D}}_u) > 0$ and $\mathrm{meas}
(\Gamma^{\mathrm{D}}_c) > 0$ for uniqueness of the solution.

%===========================================================;
%  Subsection: A model for diffusion-dependent deformation  ;
%===========================================================;
\subsection{A model for diffusion-dependent deformation}
The solid is modeled using linearized elasticity but the material 
parameters are allowed to depend on the concentration. The linearized 
strain is defined through
%-------------------------------;
%  Equation: Linearized strain  ;
%-------------------------------;
\begin{align}
  \label{Eqn:Coupled_linearized_strain}
  \mathbf{E}_l := \frac{1}{2} \left(\mathrm{grad}[\mathbf{u}] 
    + \mathrm{grad}[\mathbf{u}]^{T} \right)
\end{align}
% 
For a given concentration $c(\mathbf{x})$, the stress-strain relationship 
will be modeled as follows:  
%----------------------------------------;
%  Equation: Stress-strain relationship  ;
%----------------------------------------; 
\begin{align}
  \label{Eqn:Coupled_stress_strain}
  \mathbf{T}_c(\mathbf{u},\mathbf{x}) = \lambda(\mathbf{x},c) 
  \mathrm{tr}[\mathbf{E}_l] \mathbf{I} + 2 
  \mu(\mathbf{x},c) \mathbf{E}_l
\end{align}
%
where $\mathbf{T}_c$ is the Cauchy stress, and $\lambda$ and $\mu$ are 
the Lam\'e parameters but now can depend both on the concentration and 
position. 
%
A simple model for the Lam\'e parameters to account for degradation/healing 
of the material due to the presence of a diffusant can be taken as follows:
%--------------------------------------------;
%  Equations: Expressions for lambda and mu  ;
%--------------------------------------------;
\begin{subequations}
  \label{Eqn:Coupled_lambda_mu}
  \begin{align}
    \lambda(\mathbf{x},c) &= \lambda_0(\mathbf{x}) + \lambda_1(\mathbf{x}) 
    \frac{c(\mathbf{x})}{c_{\mathrm{ref}}} \\
    \mu(\mathbf{x},c) &= \mu_0(\mathbf{x}) + \mu_1(\mathbf{x}) 
    \frac{c(\mathbf{x})}{c_{\mathrm{ref}}} 
  \end{align}
\end{subequations}
%
where $c_{\mathrm{ref}}$ is the reference concentration (which depends on the 
problem); $\lambda_0$ and $\mu_0$ are the Lam\'e parameters for the virgin 
material (that is, in the absence of the diffusant); and $\lambda_1(\mathbf{x})$ 
and $\mu_1(\mathbf{x})$ are the weights to account for the effect of concentration 
on the Lam\'e parameters. 
%
The material parameters $\lambda_1$ and $\mu_1$ can be individually positive 
(which means that the material is healing), negative (which means that the 
material is degrading), or zero (which means that the material is unaffected 
by the presence of the diffusant). However, it is assumed that the parameters 
($\lambda_0(\mathbf{x})$, $\lambda_1(\mathbf{x})$, $\mu_0(\mathbf{x})$ and 
$\mu_1(\mathbf{x})$) and concentration are such that we have bulk modulus 
$\lambda(\mathbf{x},c) \, + \, \frac{2}{3} \mu(\mathbf{x},c) > 0$ and shear 
modulus $\mu(\mathbf{x},c) > 0$. 

The above model given by equation \eqref{Eqn:Coupled_lambda_mu} is similar 
to the concept of macroscopic damage variables, which has been introduced 
by Kachanov \cite{Kachanov_CDM} to model material damage. The basic idea 
behind the concept of macroscopic damage variables is to quantify damage 
using internal variable(s). This concept has now been widely employed in 
numerous other works on damage (for example, see the review articles by 
Chaboche \cite{1988_Chaboche_JAM_v55_p59,1988_Chaboche_JAM_v55_p65}). 
In the above model, the concentration of the diffusant can be thought as 
a macroscopic damage/healing variable. The most common criticism about 
using internal variables is that these variables (in many cases) cannot 
be measured using physical experiments. However, in the above model, the 
dependence of the Lam\'e parameters on the concentration can be measured 
indirectly by non-destructive testing methods. 

It should be noted that Weitsman \cite{2006_Weitsman_Composites_PartA_v37_p617}, 
Kringos \emph{et al}. \cite{2008_Kringos_Scarpas_Kasbergen_Selvadurai_IJPE_v9_p115,
2008_Kringos_Scarpas_Copeland_Youtcheff_IPJE_v9_p129}, and Muliana \emph{et al}. 
\cite{2009_Muliana_Rajagopal_Subramanian_JCM_v43_p1225} have considered material 
degradation as a function of concentration of the diffusant. However, the models 
developed in these works are not fully coupled. 
%
That is, the material properties of the solid are dependent on the concentration 
but the diffusivity is unaffected by the deformation of the solid. In Reference \cite{Karra_Rajagopal_degradation_arXiv_2010}, a fully coupled model is 
proposed but a specific boundary value problem (torsion of a cylindrical 
annulus undergoing degradation) is solved using the semi-inverse method. 
They did not present a computational framework, and also their mathematical 
model is different from the one present in this paper (see Remark 
\ref{Remark:Coupled_norm_of_epsilon}).

%===========================================================;
%  Subsection: A model for deformation-dependent diffusion  ;
%===========================================================;
\subsection{A model for deformation-dependent diffusion}
We define the first and second invariants of the tensor 
$\mathbf{E}_l$ as follows:
%------------------------------; 
%  Equation: Second invariant  ;
%------------------------------;
\begin{subequations}
  \label{Eqn:Coupled_second_invariant}
  \begin{align}
    I_{\mathbf{E}_l} &:= \mathrm{tr}[\mathbf{E}_l] \\
    % 
    II_{\mathbf{E}_l} &:= \sqrt{2 \, \mathrm{dev}[\mathbf{E}_l] 
      \bullet \mathrm{dev}[\mathbf{E}_l]} = \sqrt{ \frac{2}{3} 
      \left(3 \, \mathrm{tr}[\mathbf{E}^{2}_{l}] - (\mathrm{tr}
        [\mathbf{E}_l])^2 \right) } 
  \end{align}
\end{subequations}
%
where $\mathrm{dev}[\mathbf{E}_l] := \mathbf{E}_l - \frac{1}{3} \mathrm{tr}
[\mathbf{E}_l] \mathbf{I}$ is the deviatoric part of $\mathbf{E}_l$. (Note 
that the second invariant is not the principal invariant, and the reason 
for such a choice will be discussed later.) For a given strain field (that 
is, for a given deformation field), we model the effect of deformation on 
the diffusivity as follows:
%-------------------------;
%  Equation: Diffusivity  ;
%-------------------------;
\begin{align}
  \label{Eqn:Coupled_diffusivity}
  \mathbf{D}_{\mathbf{E}_l} (\mathbf{x})  = \mathbf{D}_{0}(\mathbf{x}) + 
    \left(\mathbf{D}_{T}(\mathbf{x}) - \mathbf{D}_{0}(\mathbf{x}) \right) 
  \left(\frac{\exp[\eta_T I_{\mathbf{E}_l}] - 1}{\exp[\eta_T E_{\mathrm{ref}}] - 1}\right)
  % 
  + \left(\mathbf{D}_{S}(\mathbf{x}) - \mathbf{D}_{0}(\mathbf{x}) \right) 
  \left(\frac{\exp[\eta_S II_{\mathbf{E}_l}] - 1}{\exp[\eta_S E_{\mathrm{ref}}] - 1}\right)
\end{align}
%
where $\eta_T$ and $\eta_S$ are non-negative parameters; $\mathbf{D}_0
(\mathbf{x})$, $\mathbf{D}_{T}(\mathbf{x})$ and $\mathbf{D}_{S}(\mathbf{x})$ 
are (respectively) the reference diffusivity tensors under no, tensile, and 
shear strains; and $E_{\mathrm{ref}}$ is a reference measure of the strain. 
The above model is partly motivated by the stress-induced diffusion 
experiments on glass done by McAfee \cite{McAfee_JoCP_1958_v28_p218,
McAfee_JoCP_1958_v28_p226}. These experiments have clearly shown the 
following aspects, which have been qualitatively incorporated in the 
above model.
%---------------------------------;
%  Enumerate: McAfee experiments  ;
%---------------------------------;
\begin{enumerate}[(a)]
\item The relative diffusion rate under tension is nearly five times 
  more than that of the relative diffusion rates under compression 
  and shear. 
\item The relative diffusion rate varies exponentially with 
  respect to the (circumferential) strain for Pyrex glass (see 
  \cite[Equation 15 and Figure 3]{McAfee_JoCP_1958_v28_p218}). 
\item The relative diffusion rate under compression is 
  significantly different from that of shear (see \cite[Figure 4]
  {McAfee_JoCP_1958_v28_p226}). 
\end{enumerate}
%--------------------------------------------;
%  Remark: Remark about the norm of epsilon  ;
%--------------------------------------------;
\begin{remark}
  \label{Remark:Coupled_norm_of_epsilon}
  In Reference \cite{Karra_Rajagopal_degradation_arXiv_2010}, the effect of 
  deformation on the diffusivity tensor is modeled using the Frobenius norm 
  of the Almansi-Hamel strain. (In linearized elasticity, the Almansi-Hamel 
  strain is approximately equal to linearized strain.) Although the Frobenius 
  norm of the strain is an invariant, the model cannot capture the difference 
  in diffusivity under tension, compression, and shear, which has been observed 
  in many materials. On the other hand, our model given by equation 
  \eqref{Eqn:Coupled_diffusivity} can capture such departures between the 
  diffusivities under tension, compression and shear.   	    
\end{remark}

%---------------------------------------------------;
%  Remark: Remark about principal second-invariant  ;
%---------------------------------------------------;
\begin{remark}
  A remark on the choice of invariants in the model (given by equation 
  \eqref{Eqn:Coupled_diffusivity}) is in order. Note that the second 
  principal invariant of a tensor $\mathbf{A}$ is defined as 
  \begin{align}
    II_{\mathbf{A}}^{*} := \frac{1}{2} \left( \left(\mathrm{tr}
        [\mathbf{A}]\right)^2 - \mathrm{tr}[\mathbf{A}^2] \right)
  \end{align}
  % 
  which is different from the one used in equation 
  \eqref{Eqn:Coupled_second_invariant}. It has been discussed 
  in the literature that the principal invariants are not suitable 
  to fit experimental data (e.g., Lurie \cite{Lurie_Elasticity}, 
  Anand \cite{Anand_JAM_1979_v46_p78,Anand_JMPS_1986_v34_p293}, 
  Criscione et al. \cite{Criscione_Humphrey_Douglas_Hunter_JMPS_2000_v48_p2445}, 
  Ple\v{s}ek and Kruisov\'a \cite{Plesek_Kruisova_CompStruct_2006_v84_p1141}). 
  These works employed invariants of Eulerian Hencky strain. Let the Eulerian 
  Hencky strain be denoted by $\mathbf{E}_H = \ln[\mathbf{V}]$, with $\mathbf{V}$ 
  being the left stretch tensor in the polar decomposition of the deformation 
  gradient $\mathbf{F}$. The first three invariants based on the Eulerian 
  Hencky strain which represent dilation ($k_1$), magnitude of distortion 
  ($k_2$) and mode of distortion ($k_3$) are given by 
  \begin{subequations}
    \begin{align}
      k_1 &= \mathrm{tr}[\mathbf{E}_H] = \ln[J] \\
      %
      k_2 &= \sqrt{\mathrm{dev}[\mathbf{E}_H] \bullet \mathrm{dev}[\mathbf{E}_H]} \\
      %
      k_3 &= 3\sqrt{6} \, \mathrm{det}\left[\frac{1}{k_2} \mathrm{dev}
        [\mathbf{E}_H]\right]
    \end{align}
  \end{subequations}
  % 
  where $\mathrm{dev}[\mathbf{E}_H] := \mathbf{E}_H - \frac{1}{3} 
  \mathrm{tr}[\mathbf{E}_H] \mathbf{I}$ and $J = \mathrm{det}[\mathbf{F}] \, > \, 0$. 
  For small gradients of the displacement, we have 
  \begin{align}
    \mathbf{E}_H \approx \mathbf{E}_{l}
  \end{align}
  In linearized elasticity, the constitutive equation depends only 
  on $k_1$ and $k_2$ as any dependence on $k_3$ makes the model 
  inherently non-linear (see Criscione et al. 
  \cite{Criscione_Humphrey_Douglas_Hunter_JMPS_2000_v48_p2445}).
  Herein, for modeling deformation-dependent diffusivity tensor 
  we did not use $k_3$ just to be consistent with the theory of 
  linearized elasticity. However, in the case of finite elasticity, 
  one should also use the third invariant in modeling the 
  deformation-dependent diffusivity.  
\end{remark}

One of the attractive features of the above model is that the 
parameters in the model can be established using standard 
experiments, which we shall describe below. 
%--------------------------------------------------;
%  Enumerate: Enumerate about the diffusion model  ;
%--------------------------------------------------;
\begin{enumerate}[(a)]
  \item It is easy to check that if there is no strain (that is, $\mathbf{E}_l = 
    \mathbf{0}$), then $\mathbf{D}_{\mathbf{E}_l} = \mathbf{D}_0$. Hence, one can 
    find the reference diffusivity tensor $\mathbf{D}_0$ by doing a diffusion 
    experiment on an unstrained specimen.
    % 
  \item Under simple shear, we have $I_{\mathbf{E}_l} = 0$, and 
    $II_{\mathbf{E}_l} = \alpha_S$, where $\alpha_S$ is the angle 
    of shear. As $\alpha_S \rightarrow E_{\mathrm{ref}}$, the 
    diffusivity tensor $\mathbf{D} \rightarrow \mathbf{D}_{S}$. 
    Hence, one can find $\mathbf{D}_{S}$ and $\eta_S$ by doing 
    a diffusion experiment on a specimen undergoing a simple 
    shear. 
    % 
  \item Under a uniform tri-axial tension test, the linearized strain can 
    be written as $\mathbf{E}_{l} = \alpha_T \mathbf{I}$ with $\alpha_T > 0$. 
    In this case, $II_{\mathbf{E}_l} = 0$, $I_{\mathbf{E}_l} = 3 \alpha_T$, and 
    as $\alpha_T \rightarrow \frac{1}{3} E_{\mathrm{ref}}$ we have $\mathbf{D} 
    \rightarrow \mathbf{D}_{T}$. Hence, one can find $\mathbf{D}_{T}$ and 
    $\eta_T$ in the model given by equation \eqref{Eqn:Coupled_diffusivity} 
    by doing a diffusion experiment on a specimen under uniform tri-axial 
    strain. 
    
    There are experimental techniques discussed in the literature for 
    maintaining a specimen under uniform tri-axial strain. To name 
    a few, tri-axial tensile testing of brittle materials such as 
    calestone (a dental plaster), copper and aluminum alloys, 
    austenitic stainless steel were described by Cridland and 
    Wood \cite{Cridland_Wood_IJFM_1968_v4_p277}, Hayhurst and 
    Felce \cite{Hayhurst_Felce_EFM_1986_v25_p645} and Calloch 
    and Marquis \cite{Calloch_Marquis_IJP_1999_v15_p521}. 
    Advanced tri-axial testing of geomaterials such as rock and 
    soil were carried out by Donaghe \emph{et al}. \cite{Donaghe_Chaney_Marshall}, 
    Hunsche \cite{Cristescu_Gioda} and Wawersik 
    \cite{1997_Wawersik_Carlson_Holcomb_Williams_IJRMMS_v34_p330}.
    %
    Despite these experimental techniques, it can well be argued that 
    maintaining a specimen under uniform tri-axial strain can be a 
    difficult and expensive. 
    %
    In that case, after determining $\mathbf{D}_0$, $\mathbf{D}_{S}$ 
    and $\eta_S$ one can evaluate $\mathbf{D}_{T}$ and $\eta_T$ using 
    either uni-axial or bi-axial tension tests. However, in uni-axial 
    and bi-axial tests, it should be noted that $II_{\mathbf{E}_l}$ will 
    not be equal to zero.
  % 
\end{enumerate}

%-----------------------------------------------;
%  Remark: Diffusivity Tensor from compression  ;
%-----------------------------------------------;
\begin{remark}
  For brittle materials such as concrete, ceramics, metallic alloys and 
  geomaterials such as soil and rock it is relatively easier to perform 
  compression tests than tension tests. In those cases, the expression 
  for diffusivity tensor $\mathbf{D}_{\mathbf{E}_l} (\mathbf{x})$ can be 
  modeled as follows:
%-------------------------------------------------;
%  Equation: Diffusivity in Compression and shear ;
%-------------------------------------------------;
\begin{align}
  \label{Eqn:Coupled_diffusivity_compression}
  \mathbf{D}_{\mathbf{E}_l} (\mathbf{x})  = \mathbf{D}_{0}(\mathbf{x}) + 
    \left(\mathbf{D}_{0}(\mathbf{x}) - \mathbf{D}_{C}(\mathbf{x}) \right) 
  \left(\frac{\exp[\eta_C I_{\mathbf{E}_l}] - 1}{\exp[\eta_C E_{\mathrm{ref}}] - 1}\right)
  % 
  + \left(\mathbf{D}_{S}(\mathbf{x}) - \mathbf{D}_{0}(\mathbf{x}) \right) 
  \left(\frac{\exp[\eta_S II_{\mathbf{E}_l}] - 1}{\exp[\eta_S E_{\mathrm{ref}}] - 1}\right)
\end{align}
%
where $\eta_C$ and $\eta_S$ are non-negative parameters; $\mathbf{D}_0
(\mathbf{x})$, $\mathbf{D}_{C}(\mathbf{x})$, and $\mathbf{D}_{S}(\mathbf{x})$ 
are (respectively) reference diffusivity tensors under no, compressive, and 
shear strains. Also, it should be noted that modeling diffusivity as an 
exponential function of stress/strain is quite popular in literature (e.g., 
see McAfee \cite{McAfee_JoCP_1958_v28_p218},  Fahmy and Hurt 
\cite{1980_Fahmy_Hurt_PC_v1_p77}).
\end{remark}

The diffusivity tensor is assumed to be symmetric, bounded, 
and uniformly elliptic. That is, 
%---------------------------;
%  Equation: Symmetry of D  ;
%---------------------------;
\begin{align}
  \mathbf{D}_{\mathbf{E}_l}(\mathbf{x}) = \mathbf{D}_{\mathbf{E}_l}^{T} 
  (\mathbf{x}) \quad \forall \; \mathbf{x} \in \Omega 
\end{align}
%
and there exists two constants $0 < \xi_1 \leq \xi_2 < +\infty$ such that 
%--------------------------------;
%  Equation: Positive constants  ;
%--------------------------------;
\begin{align}
  \xi_1 \mathbf{y}^{T} \mathbf{y} \leq \mathbf{y}^{T} \mathbf{D}_{\mathbf{E}_l}
  (\mathbf{x}) \mathbf{y} \leq \xi_2 \mathbf{y}^{T} \mathbf{y}  \quad \forall 
  \; \mathbf{x} \in \Omega \; \; \mathrm{and} \; \; \forall \; \mathbf{y} \in 
  \mathbb{R}^{nd}
\end{align}

%=========================================;
%  Subsection: Governing field equations  ;
%=========================================;
\subsection{Governing field equations }
The governing equations for the deformation of the solid 
can be written as follows: 
%-----------------------------------;
%  Equation: Deformation equations  ;
%-----------------------------------;
\begin{subequations}
  \label{Eqn:Coupled_deformation_equations}
  \begin{align}
    &\mathrm{div}[\mathbf{T}_c] + \rho(\mathbf{x}) \mathbf{b}
    (\mathbf{x}) = \mathbf{0} \quad \mathrm{in} \; \Omega \\
    %
    &\mathbf{u}(\mathbf{x}) = \mathbf{u}^{\mathrm{p}} (\mathbf{x}) 
    \quad \mathrm{on} \; 
    \Gamma^{\mathrm{D}}_{u} \\
    % 
    &\mathbf{T}_c \, \mathbf{n}(\mathbf{x}) = \mathbf{t}^{\mathrm{p}} 
    (\mathbf{x}) \quad \mathrm{on} \; \Gamma^{\mathrm{N}}_{u} 
  \end{align}
\end{subequations}
% 
where $\rho(\mathbf{x})$ is the density, $\mathbf{b}(\mathbf{x})$ is 
the specific body force, $\mathbf{u}^{\mathrm{p}}(\mathbf{x})$ is the 
prescribed displacement, $\mathbf{t}^{\mathrm{p}}(\mathbf{x})$ is the 
prescribed traction, and recall that $\mathbf{n}(\mathbf{x})$ is the 
unit outward normal to the boundary. In the absence of internal couples, 
the balance of angular momentum reads 
%-----------------------------------------;
%  Equation: Balance of angular momentum  ;
%-----------------------------------------;
\begin{align}
  \label{Eqn:Coupled_angular_momentum}
  \mathbf{T}_c = \mathbf{T}^{T}_c
\end{align}
%
which the Cauchy stress given in equation 
\eqref{Eqn:Coupled_stress_strain} clearly satisfies. The governing 
equations for the steady-state (deformation-dependent) diffusion 
process can be written as follows:
%--------------------------------------------;
%  Equation: Steady-State Diffusion process  ;
%--------------------------------------------;
\begin{subequations}
  \label{Eqn:Coupled_diffusion_equations}
  \begin{align}
    -&\mathrm{div}\left[ \mathbf{D}_{\mathbf{E}_l}(\mathbf{x}) \, 
      \mathrm{grad}[c]\right] = f(\mathbf{x}) \quad \mathrm{in} 
    \; \Omega \\
    % 
    &c(\mathbf{x}) = c^{\mathrm{p}}(\mathbf{x}) \quad \mathrm{on} 
    \; \Gamma^{\mathrm{D}}_{c} \\
    %
    &\mathbf{n}(\mathbf{x}) \cdot \mathbf{D}_{\mathbf{E}_l}
    (\mathbf{x}) \, \mathrm{grad}[c] = h^{\mathrm{p}}(\mathbf{x}) 
    \quad \mathrm{on} \; \Gamma^{\mathrm{N}}_{c}
  \end{align}
\end{subequations}
%
where $c^{\mathrm{p}}(\mathbf{x})$ is the prescribed concentration, 
$h^{\mathrm{p}}(\mathbf{x})$ is the prescribed concentration flux 
on the boundary, and $f(\mathbf{x})$ is the volumetric source. 

It is easy to see that the governing equations for the deformation 
\eqref{Eqn:Coupled_deformation_equations} and the governing equations 
for the diffusion \eqref{Eqn:Coupled_diffusion_equations} are coupled 
through equations \eqref{Eqn:Coupled_stress_strain} and \eqref{Eqn:Coupled_diffusivity}. 
%
To predict the degradation/healing of the solid due to the diffusant, 
one needs to solve this system of coupled nonlinear partial differential 
equations given by equations 
\eqref{Eqn:Coupled_linearized_strain}-\eqref{Eqn:Coupled_second_invariant}, 
\eqref{Eqn:Coupled_diffusivity}, \eqref{Eqn:Coupled_deformation_equations} 
and \eqref{Eqn:Coupled_diffusion_equations}. It is noteworthy that, except 
for simple problems, it is not possible to find analytical solutions to this 
system of equations, and one needs to resort to numerical solutions for 
solving realistic and practical problems. 

However, to obtain reliable and predictive numerical solutions, one 
has to overcome many numerical challenges.  In particular, one has 
to make sure that the chosen numerical scheme gives non-negative 
values for the concentration as a negative value for the concentration 
is unphysical. We will show in a subsequent section that the classical 
single-field formulation produces negative concentrations. This is 
particularly true if the medium is anisotropic, and one may even 
get negative values for the concentration even when the medium is 
isotropic if the mesh is not chosen with care. For example, one 
need to choose a mesh with square elements or a well-centered 
triangular mesh \cite{Nakshatrala_Valocchi_JCP_2009_v228_p6726} 
even for isotropic diffusion. (In two-dimensions a well-centered 
triangular mesh means that all the angles of any triangle are 
acute. Similarly, one can define a well-centered mesh in higher 
dimensions \cite{Vanderzee_Hirani_Guoy_Ramos_2008}.)

\emph{We now present a numerical framework to solve the coupled 
deformation-diffusion equations \eqref{Eqn:Coupled_linearized_strain}
--\eqref{Eqn:Coupled_diffusion_equations} in a systematic manner.} 

==> Sections/S3_Coupled_Computational_framework.tex <==
%************************************************;
%                                                ;
%  NAME                                          ;
%    S3_Coupled_Computational_framework.tex      ;
%                                                ;
%************************************************;
\section{A COUPLED COMPUTATIONAL FRAMEWORK}
\label{Sec:Coupled_Computational_framework}
%
The computational framework will be based on the Finite Element 
Method (FEM), convex quadratic programming, and staggered coupling 
techniques. To this end, let the domain $\Omega$ be decomposed into 
``$Nele$'' non-overlapping open sub-domains (which in the finite 
element context will be elements). That is, 
%-----------------------------------------;
%  Equation: Decomposition into elements  ;
%-----------------------------------------;
\begin{align}
  \bar{\Omega} = \bigcup_{e = 1}^{Nele} \bar{\Omega}^{e}
\end{align}
%
where a superposed bar denotes the set closure. The boundary of $\Omega^e$ 
is denoted as $\partial \Omega^{e} := \bar{\Omega}^{e} - \Omega^{e}$. For 
convenience and to avoid errors due to projection operators, we shall 
employ the same computational mesh for both deformation and diffusion 
analyses. (Note that one needs to employ projection operators if different 
computational meshes are employed for multi-field problems like coupled 
deformation-diffusion.) We now present individual solvers for deformation 
and diffusion, and a coupling algorithm to couple individual solvers to 
obtain the coupled response. The solver for the diffusion problem will 
always give physically meaningful non-negative values for the concentration.

%===========================================================;
%  Subsection: A numerical solver for deformation analysis  ;
%===========================================================;
\subsection{A numerical solver for deformation analysis}
\label{Sec:Coupled_Numerical_deformation}
For solving the pure deformation problem (that is, for a given 
concentration field) the computational framework utilizes the 
standard single-field (pure displacement) formulation. However, 
it should be noted that one can employ any other formulation 
(e.g., B-bar method \cite{Hughes_IJNME_1980_v15_p1413}, stabilized 
mixed formulation 
\cite{Nakshatrala_Masud_Hjelmstad_CompMech_2008_v41_p547}, 
mixed assumed strain formulation \cite{Simo_Rifai_IJNME_1990_v29_p1595}, 
mixed enhanced formulation \cite{Taylor_IJNME_2000_v47_p205}) to solve 
the (pure) deformation problem. For completeness, we shall 
now briefly outline the single-field formulation. To this 
end, we shall define the following function spaces:
%-----------------------------;
%  Equation: Function spaces  ;
%-----------------------------;
\begin{subequations}
  \begin{align}
    \mathcal{U} &:= \left\{\mathbf{u}(\mathbf{x}) \in 
      \left(H^{1}(\Omega)\right)^{nd} \; \big| \; \mathbf{u}
      (\mathbf{x}) = \mathbf{u}^{\mathrm{p}}(\mathbf{x}) \; 
      \mathrm{on} \; \Gamma^{\mathrm{D}}_{u} \right\} \\
    % 
    \mathcal{W} &:= \left\{\mathbf{w}(\mathbf{x}) \in 
      \left(H^{1}(\Omega)\right)^{nd} \; \big| \; \mathbf{w}
      (\mathbf{x}) = \mathbf{0} \; \mathrm{on} \; 
      \Gamma^{\mathrm{D}}_{u} \right\} 
  \end{align}
\end{subequations}
% 
where $H^{1}(\Omega)$ is a standard Sobolev space on $\Omega$ 
\cite{Brezzi_Fortin}, and recall that ``$nd$" is the number 
of spatial dimensions. The standard single-field formulation 
for the pure deformation problem \eqref{Eqn:Coupled_deformation_equations} 
reads: Find $\mathbf{u}(\mathbf{x}) \in \mathcal{U}$ such that we have
%--------------------------------------;
%  Equation: Single field formulation  ;
%--------------------------------------;
\begin{align}
  \label{Eqn:Coupled_single_field_formulation_deformation}
  \mathcal{B}_{u}(\mathbf{w};\mathbf{u}) = L_{u}(\mathbf{w}) 
  \quad \forall \; \mathbf{w}(\mathbf{x}) \in \mathcal{W}
\end{align}
%
where the bilinear form and linear functional are, 
respectively, defined as follows:
%-------------------------------------------------;
%  Equation: Bilinear form and linear functional  ;
%-------------------------------------------------;
\begin{subequations}
  \begin{align}
    \mathcal{B}_{u}(\mathbf{w};\mathbf{u}) &:= \int_{\Omega} 
    \mathrm{grad}[\mathbf{w}] \bullet \mathbf{T}_c(\mathbf{u}, 
    \mathbf{x}) \; \mathrm{d} \Omega \\
    %
    L_{u}(\mathbf{w}) &:= \int_{\Omega} \mathbf{w}(\mathbf{x}) 
    \cdot \rho(\mathbf{x}) \mathbf{b}(\mathbf{x}) \; \mathrm{d} 
    \Omega + \int_{\Gamma^{\mathrm{N}}_{u}} \mathbf{w}(\mathbf{x}) 
    \cdot \mathbf{t}^{\mathrm{p}}(\mathbf{x}) \; \mathrm{d} \Gamma 
  \end{align}
\end{subequations}
% 
For a non-negative integer $m$, let $\mathbb{P}^{m}(\Omega^{e})$ 
denotes the linear vector space spanned by polynomials up-to 
$m$th order defined on the sub-domain $\Omega^{e}$. We shall 
define the following finite dimensional subsets of $\mathcal{U}$ 
and $\mathcal{W}$: 
%----------------------------------------------------------;
%  Equation: Finite dimensional subspaces for deformation  ;
%----------------------------------------------------------;
\begin{subequations}
  \begin{align}
    \mathcal{U}^{h} &:= \left\{\mathbf{u}^{h}(\mathbf{x}) 
      \in \mathcal{U} \; \big| \; \mathbf{u}^{h}(\mathbf{x}) 
      \in \left(C^{0}(\bar{\Omega})\right)^{nd} , \, \mathbf{u}^{h}
      (\mathbf{x}) \big|_{\Omega^e} \in \left(\mathbb{P}^{k}
        (\Omega^{e})\right)^{nd}, \, e = 1, \cdots, Nele \right\} \\
    % 
    \mathcal{W}^{h} &:= \left\{\mathbf{w}^{h}(\mathbf{x}) \in 
      \mathcal{W} \; \big| \; \mathbf{w}^{h}(\mathbf{x}) \in 
      \left(C^{0}(\bar{\Omega})\right)^{nd}, \, \mathbf{w}^{h}
      (\mathbf{x}) \big|_{\Omega^e} \in \left(\mathbb{P}^{k}
        (\Omega^{e})\right)^{nd}, \, e = 1, \cdots, Nele \right\}        
  \end{align}
\end{subequations}
% 
where $k$ is a non-negative integer. A corresponding finite element 
formulation for the deformation analysis can be written as: Find 
$\mathbf{u}^{h}(\mathbf{x}) \in \mathcal{U}^{h}$ such that we have
%--------------------------------------------------------;
%  Equation: Finite element formulation for deformation  ;
%--------------------------------------------------------;
\begin{align}
  \mathcal{B}_{u}(\mathbf{w}^{h};\mathbf{u}^{h}) = L_{u}(\mathbf{w}^{h}) 
  \quad \forall \; \mathbf{w}^{h}(\mathbf{x}) \in \mathcal{W}^{h}
\end{align}
%
After the finite element discretization, the deformation analysis 
will involve solving the following discrete equations:
%-------------------------------------------------;
%  Equation:  Discrete equations for deformation  ;
%-------------------------------------------------;
\begin{align}
  \boldsymbol{K}_u(\boldsymbol{c}) \boldsymbol{u} = \boldsymbol{f}_u
\end{align} 
%
where $\boldsymbol{u}$ denotes the nodal displacements, $\boldsymbol{c}$ 
denotes the nodal concentrations, and the stiffness matrix for the 
deformation analysis $\boldsymbol{K}_u$ depends on the concentration 
of the diffusant. 

%================================================;
%  Subsection: A numerical solver for diffusion  ;
%================================================;
\subsection{A numerical solver for diffusion analysis}
\label{Subsec:Coupled_solver_for_diffusion}
Before we provide a numerical solver for diffusion, we shall provide a 
mathematical argument to show that $c(\mathbf{x}) \geq 0$ in $\Omega$ 
even for the coupled problem. We shall assume that a solution exists 
for the coupled problem. (Proving existence of a solution for the 
coupled system is a research topic by itself, and is beyond the scope 
of this paper. However, in this paper we do find a numerical solution 
for various coupled deformation-diffusion problems.) That is, there 
exists a pair, $\mathbf{u}(\mathbf{x})$ and $c(\mathbf{x})$, such 
that they satisfy the coupled system of equations. For the given 
displacement field, $\mathbf{u}(\mathbf{x})$, (and hence for a given 
strain field $\mathbf{E}_l(\mathbf{x})$) we define 
\begin{align}
  \mathbf{D}(\mathbf{x}) := \mathbf{D}_{\mathbf{E}_l}(\mathbf{x})
\end{align}
%
From the theory of partial differential equations we have the 
following maximum principle \cite{Evans_PDE}: 
%-----------------------------------------;
%  Theorem: Continuous maximum principle  ;
%-----------------------------------------;
\begin{theorem}
  \label{Thm:Continuous_maximum_principle}
  Let $c^{\mathrm{p}}(\mathbf{x}) \geq 0$ on $\partial \Omega$ 
  and $\mathbf{D}(\mathbf{x})$ be continuously differentiable. 
  If $c(\mathbf{x}) \in C^{2}(\Omega) \cap C^{0}(\bar{\Omega})$ 
  satisfies the differential inequality $-\mathrm{div}[
  \mathbf{D}(\mathbf{x})\mathrm{grad}[c]] = f(\mathbf{x}) 
  \geq 0$ in $\Omega$, then we have the following non-negative 
  property: 
  \begin{align}
    c(\mathbf{x}) \geq 0 \quad \mathrm{in} \; \bar{\Omega}
  \end{align}
\end{theorem}

%------------------------------------------;
%  Remark: Remark about weaker regularity  ;
%------------------------------------------;
\begin{remark}
  The above maximum principle theorem is due to Hopf, and a proof 
  can be found in any standard textbook on partial differential 
  equations (e.g., References \cite{McOwen,Evans_PDE,Protter_Weinberger,
    Gilbarg_Trudinger,Han_Lin}). One can find in the literature maximum 
  principles for diffusion-type equations under weaker regularity than 
  $C^{2}(\Omega) \cap C^{0}(\bar{\Omega})$ (for example, see References 
  \cite{Mazja_Plamenevskii_TMMS_1980_v1_p49,Borsuk_Kondratiev}). But 
  such a thorough treatment is beyond the scope of this paper, and 
  is not crucial to our presentation. 
\end{remark}

As discussed earlier, many existing numerical formulations (including 
the single-field formulation, which is based on the Galerkin principle) 
for diffusion-type equation do not meet the non-negative constraint. 
For example, the widely used single-field formulation (which is based 
on the Galerkin principle) does not produce physically meaningful 
non-negative solutions. 
%
We now present a novel methodology of enforcing the non-negative 
constraint on the concentration of the diffusant. The methodology 
works well for general computational grids and for low-order finite 
elements. 

We start with the single-field formulation, and then modify the 
underlying (discrete) variational statement to meet the non-negative 
constraint.  We shall define the following function spaces 
%-----------------------------;
%  Equation: Function spaces  ;
%-----------------------------;
\begin{subequations}
  \begin{align}
    \mathcal{P} &:= \left\{c(\mathbf{x}) \in H^{1}(\Omega) \; \big| \; c(\mathbf{x}) = 
      c^{\mathrm{p}}(\mathbf{x}) \; \mathrm{on} \; \Gamma^{\mathrm{D}}_{c}\right\} \\
    \mathcal{Q} &:= \left\{q(\mathbf{x}) \in H^{1}(\Omega) \; \big| \; q(\mathbf{x}) = 0 \; 
  \mathrm{on} \; \Gamma^{\mathrm{D}}_{c}\right\} 
\end{align}
\end{subequations}
%
where $H^{1}(\Omega)$ is a standard Sobolev space \cite{Brezzi_Fortin}. 
We also relax the regularity of the diffusivity tensor for weak solutions, 
and assume that  
%------------------------------------;
%  Equation: D is square integrable  ;
%------------------------------------;
\begin{align}
  \int_{\Omega} \mathrm{tr}[\mathbf{D}_{\mathbf{E}_l}(\mathbf{x})^{T} 
  \mathbf{D}_{\mathbf{E}_l} (\mathbf{x})] \; \mathrm{d} \Omega < +\infty
\end{align}
%
where $\mathrm{tr}[\cdot]$ is the standard trace operator used 
in tensor algebra and continuum mechanics \cite{Chadwick}. The 
standard single field formulation for tensorial diffusion equation 
\eqref{Eqn:Coupled_diffusion_equations} reads: Find $c(\mathbf{x}) 
\in \mathcal{P}$ such that we have
%--------------------------------------;
%  Equation: Single field formulation  ;
%--------------------------------------;
\begin{align}
  \label{Eqn:Coupled_single_field_formulation_diffusion}
  \mathcal{B}_{c}(q;c) = L_{c}(q) \quad \forall \; 
  q(\mathbf{x}) \in \mathcal{Q}
\end{align}
%
where the bilinear form and linear functional are, respectively, 
defined as 
%-------------------------------------------------;
%  Equation: Bilinear form and linear functional  ;
%-------------------------------------------------;
\begin{subequations}
  \begin{align}
    \mathcal{B}_{c}(q;c) &:= \int_{\Omega} \mathrm{grad}[q] \cdot 
    \mathbf{D}_{\mathbf{E}_l}(\mathbf{x}) \mathrm{grad}[c] \; 
    \mathrm{d} \Omega \\
    % 
    L_{c}(q) &:= \int_{\Omega} q(\mathbf{x}) \; f(\mathbf{x}) \; 
    \mathrm{d} \Omega + \int_{\Gamma^{\mathrm{N}}_{c}} q(\mathbf{x}) 
    \; h^{\mathrm{p}}(\mathbf{x}) \; \mathrm{d} \Gamma 
  \end{align}
\end{subequations}
%
It is well-known that the above weak form 
\eqref{Eqn:Coupled_single_field_formulation_diffusion} 
has a corresponding variational statement, which can be 
written as follows:
%-----------------------------------;
%  Equation: Variational statement  ;
%-----------------------------------; 
\begin{align}
  \mathop{\mathrm{minimize}}_{c(\mathbf{x}) \in \mathcal{P}} 
  \quad \frac{1}{2} \mathcal{B}_{c}(c;c) - L_{c}(c)
\end{align}
%
We shall define the following finite dimensional vector spaces 
of $\mathcal{P}$ and $\mathcal{Q}$:
%------------------------------------------;
%  Equation: Finite dimensional subspaces  ;
%------------------------------------------;
\begin{subequations}
  \begin{align}
    \mathcal{P}^{h} &:= \left\{c^{h}(\mathbf{x}) \in \mathcal{P} \; 
      \big| \; c^{h}(\mathbf{x})  \in C^{0}(\bar{\Omega}), \, c^{h}
      (\mathbf{x}) \big|_{\Omega^e} \in \mathbb{P}^{k}(\Omega^{e}), \, 
      e = 1, \cdots, Nele \right\} \\
    % 
    \mathcal{Q}^{h} &:= \left\{q^{h}(\mathbf{x}) \in \mathcal{Q} 
      \; \big| \; q^{h}(\mathbf{x}) \in C^{0}(\bar{\Omega}), \, q^{h}
      (\mathbf{x}) \big|_{\Omega^e} \in \mathbb{P}^{k}(\Omega^{e}),  \, 
      e = 1, \cdots, Nele \right\}       
  \end{align}
\end{subequations}
% 
where $k$ is a non-negative integer. (Recall that, for a non-negative 
integer $m$, $\mathbb{P}^{m}(\Omega^{e})$ denotes the linear vector 
space spanned by polynomials up-to $m$th order defined on the subdomain 
$\Omega^{e}$.) A corresponding finite element formulation can be written 
as: Find $c^{h}(\mathbf{x}) \in \mathcal{P}^{h}$ such that we have 
%-----------------------------------------------------;
%  Equation: Single field finite element formulation  ;
%-----------------------------------------------------;
\begin{align}
  \label{Eqn:Coupled_single_field_FE_formulation}
  \mathcal{B}_{c}(q^{h};c^{h}) = L_{c}(q^{h}) \quad \forall \; 
  q^{h}(\mathbf{x}) \in \mathcal{Q}^{h}
\end{align}

%======================================================================;
%  Subsection: A non-negative solver for tensorial diffusion equation  ;
%======================================================================;
\subsubsection{A non-negative solver for tensorial diffusion equation}
\label{Subsubec:Coupled_Non-negative}
We shall use the symbols $\preceq$ and $\succeq$ to denote component-wise 
inequalities for vectors. That is, for given any two (finite dimensional) 
vectors $\boldsymbol{a}$ and $\boldsymbol{b}$ 
%-----------------------------------------;
%  Equation: Definition of preceq symbol  ;
%-----------------------------------------;
\begin{align}
  \boldsymbol{a} \preceq \boldsymbol{b} \quad \mbox{means that } 
  \quad a_i \leq b_i \; \forall \; i
\end{align}
%
Similarly, one can define the symbol $\succeq$. We shall denote the 
standard inner-product on Euclidean spaces by $\langle \cdot;\cdot 
\rangle$.

After finite element discretization, for given nodal displacement 
vector $\boldsymbol{u}$, the discrete equation for the diffusion 
analysis takes the following form:
%------------------------------------------------------------;
%  Equation: Discretization equation for diffusion equation  ;
%------------------------------------------------------------;
\begin{align}
  \label{Eqn:Coupled_discrete_diffusion}
  \boldsymbol{K}_c(\boldsymbol{u}) \boldsymbol{c} = \boldsymbol{f}_c
\end{align}
% 
where $\boldsymbol{K}_c$ is a symmetric positive definite matrix, 
$\boldsymbol{c}$ is the vector containing nodal concentrations, 
and $\boldsymbol{f}_c$ is the source vector. Let ``$ndofs$'' 
denote the number of degrees-of-freedom for the concentration. 
The matrix $\boldsymbol{K}_c$ is of size $ndofs \times ndofs$, 
and the vectors $\boldsymbol{c}$ and $\boldsymbol{f}_c$ are of 
size $ndofs \times 1$. The finite element discretized equation 
\eqref{Eqn:Coupled_discrete_diffusion} is \emph{equivalent} to 
the following minimization problem:
%---------------------------------------------------------;
%  Equation: Minimization problem for diffusion analysis  ;
%---------------------------------------------------------;
\begin{align}
  \label{Eqn:Coupled_diffusion_minimization}
  \mathop{\mbox{minimize}}_{\boldsymbol{c} \in \mathbb{R}^{ndofs}} 
  \quad  \frac{1}{2} \langle \boldsymbol{c}; \boldsymbol{K}_c(\boldsymbol{u})
  \boldsymbol{c}\rangle - \langle\boldsymbol{c};\boldsymbol{f}_c\rangle 
\end{align}
% 
As shown in Figure \ref{Fig:Plate_with_hole_concentration_Galerkin}, the 
numerical formulation based on equations \eqref{Eqn:Coupled_discrete_diffusion}  
and \eqref{Eqn:Coupled_diffusion_minimization} produces unphysical negative 
concentrations for many practically important problems. (More examples showing 
Galerkin formulation producing negative solutions can be found in Reference 
\cite{Nagarajan_Nakshatrala_IJNMF_2010}.) Following the ideas outlined in 
References \cite{Nakshatrala_Valocchi_JCP_2009_v228_p6726,
Liska_Shashkov_CiCP_2008_v3_p852,Nagarajan_Nakshatrala_IJNMF_2010} 
a non-negative formulation corresponding to 
\eqref{Eqn:Coupled_diffusion_minimization} can be written as follows:
%--------------------------------------;
%  Equation: Non-negative formulation  ;
%--------------------------------------;
\begin{subequations}
  \label{Eqn:Coupled_diffusion_non-negative}
  \begin{align}
    \mathop{\mbox{minimize}}_{\boldsymbol{c} \in \mathbb{R}^{ndofs}} & 
    \quad \frac{1}{2} \langle \boldsymbol{c};\boldsymbol{K}_c(\boldsymbol{u}) 
    \boldsymbol{c}\rangle - \langle\boldsymbol{c};\boldsymbol{f}_c\rangle \\
    % 
    \mbox{subject to} & \quad \boldsymbol{c} \succeq \boldsymbol{0} 
  \end{align}
\end{subequations}
%
Since for a given nodal displacement vector, the matrix $\boldsymbol{K}_c
(\boldsymbol{u})$ is positive definite, the above problem 
\eqref{Eqn:Coupled_diffusion_non-negative} belongs to convex quadratic 
programming. From optimization theory it can be shown that the problem 
\eqref{Eqn:Coupled_diffusion_non-negative} has a unique global minimizer. 
There are many robust numerical algorithms available in the literature to 
solve the aforementioned constrained minimization problem (e.g., active 
set strategy, interior point methods, barrier methods). In all our numerical 
simulations, we have employed the active set strategy. A detailed discussion 
on numerical optimization can be found in references \cite{Nocedal_Wright,
Boyd_convex_optimization,Mangasarian}. 

%==============================================;
%  Subsection: A staggered coupling algorithm  ;
%==============================================;
\subsection{A staggered coupling algorithm}
\label{Sec:Coupled_Coupling_algorithm}
Current coupling algorithms are broadly classified into main 
classes: monolithic and staggered schemes. In \emph{monolithic 
  schemes} discretization scheme is applied to the full problem. 
On the other hand, in \emph{staggered schemes} (which are based 
on operator-split techniques) the coupled system is partitioned, 
often according to the different coupled fields (in our case, 
concentration and displacement in deformation-diffusion analysis), 
and each partition is treated by different and tailored numerical 
schemes. There is no easy way to incorporate our non-negative 
formulation within a monolithic scheme. Therefore, we shall 
employ a staggered coupling approach. The various steps of 
the proposed coupling algorithm is presented in Algorithm 
\ref{Algo:Coupled_fixed_point}.
 
%------------------------------------------------------------------------------;
%  Algorithm: Staggered coupling algorithm for deformation-diffusion analysis  ;
%------------------------------------------------------------------------------;
\begin{algorithm}              
  \caption{Staggered coupling algorithm for deformation-diffusion analysis}          
  \label{Algo:Coupled_fixed_point}                          
  \begin{algorithmic}[1]                   
    % 
    \STATE Input: tolerance ($\epsilon_{\mathrm{TOL}}^{(c)}$), maximum 
    number of iteration (MAXITERS)
    % 
    \STATE Guess $\boldsymbol{c}^{(0)} \succeq \boldsymbol{0}$
    \FOR{$i = 1, 2, \cdots$}
    % 
    \IF {$i > \mathrm{MAXITERS}$}
    \STATE Solution did not converge in specified maximum number of 
    iterations. EXIT
    \ENDIF
    % 
    \STATE Call deformation solver: Obtain $\boldsymbol{u}^{(i)}$ by solving 
    \begin{align*}
      \boldsymbol{K}_{u} (\boldsymbol{c}^{(i - 1)}) \boldsymbol{u}^{(i)} = 
      \boldsymbol{f}_u
    \end{align*}
    % 
    \STATE Call non-negative diffusion solver: Obtain $\boldsymbol{c}^{(i)}$ 
    by solving the following minimization problem
    \begin{align*}
      \mathop{\mathrm{minimize}}_{\boldsymbol{c}^{(i)} \in \mathbb{R}^{ndofs}} &\quad \frac{1}{2} 
      \langle \boldsymbol{c}^{(i)};\boldsymbol{K}_{c} (\boldsymbol{u}^{(i)}) 
      \boldsymbol{c}^{(i)}\rangle - \langle\boldsymbol{c}^{(i)}; 
      \boldsymbol{f}_c \rangle \\
      % 
      \mbox{subject to} &\quad \boldsymbol{c}^{(i)} \succeq \boldsymbol{0}
    \end{align*}
    % 
    \IF{$\| \boldsymbol{c}^{(i)} - \boldsymbol{c}^{(i - 1)}\| < 
      \epsilon_{\mathrm{TOL}}^{(c)}$} 
    \STATE Staggered scheme converged. EXIT
    \ENDIF
    \ENDFOR
  \end{algorithmic}
\end{algorithm}

%------------------------------------------;
%  Remark: Norm in the stopping criterion  ;
%------------------------------------------;
\begin{remark}
  In this paper, we shall use the 2-norm in the stopping 
  criterion $\|\boldsymbol{c}^{(i)} - \boldsymbol{c}^{(i-1)}\| 
  < \epsilon^{(c)}_{\mathrm{TOL}}$ in the staggered coupling 
  algorithm. However, one could use any other norm as in 
  (finite dimensional) Euclidean spaces all norms are 
  \emph{equivalent} \cite{Halmos}.
\end{remark}

%----------------------------------;
%  Remark: Algorithm is staggered  ;
%----------------------------------;
\begin{remark}
  It should be noted that even though the solution procedure 
  is a staggered scheme, the problem is coupled, and the 
  converged numerical solution will be the coupled response. 
\end{remark}

==> Sections/S4_P1.tex <==
%********************************************;
%                                            ;
%  NAME                                      ;
%    S4_Coupled_Numerical_results.tex        ;
%                                            ;
%********************************************;
\section{PERFORMANCE OF THE PROPOSED FRAMEWORK}
\label{Sec:Coupled_Numerical_results}
%
In this section, we present numerical solutions of several realistic 
problems using the proposed mathematical model and computational 
framework. The first set of problems involve degradation/healing 
of beams, and the second set involves degradation/healing of 
rectangular domains with holes. All these problems naturally 
arise in many important engineering applications. For example, 
study of degradation of beams is important to assess the 
performance of structural components in bridges, towers, 
buildings and aircraft wings. 
%
The second set of problems is to study the degradation of ducts 
carrying chemicals (e.g., water, carbon-dioxide, coolant) cutting 
through a slab or a wall, which have many applications in civil and nuclear 
structures. Using these two sets of representative problems we 
will illustrate the performance of the proposed computational framework 
for coupled deformation-diffusion analyses. In particular, we will show 
that the proposed computational framework produces physical and reliable 
solutions. We also systematically study the effect of the concentration 
of the diffusant on the deformation of the solid and vice-versa.

%\begin{remark}
%\label{Rem:Diffusivity_Assumed}
Here, in these representative numerical examples we have chosen
$\mathbf{D}_0$, $\mathbf{D}_T$ and $\mathbf{D}_S$ as follows: 
%
\begin{subequations}
 \label{Eqn:Representative_D0_DT_DS}
  \begin{align}
  %%
  \mathbf{D}_0 &= 
  \left(\begin{array}{cc}
  \cos(\theta) & -\sin(\theta) \\ 
  \sin(\theta) & \cos(\theta)
  \end{array}\right)
  %
  \left(\begin{array}{cc}
  d_1 & 0 \\ 
  0 & d_2
  \end{array}\right)
  %
  \left(\begin{array}{cc}
  \cos(\theta) & \sin(\theta) \\ 
  -\sin(\theta) & \cos(\theta)
  \end{array}\right) \\
  %%
  \mathbf{D}_T &= \Phi_T\mathbf{D}_0 \\
  %%
  \mathbf{D}_S &= \Phi_S\mathbf{D}_0
  %%
  \end{align}
\end{subequations}
%
where $\Phi_T$ and $\Phi_S$ are some positive real numbers. 
The reason for choosing such a form is that a change in each
of the $\mathbf{D}_T$ and $\mathbf{D}_S$ effect the concentration
in a considerable manner in various important realistic problems. 
But in general each component of $\mathbf{D}_T$, $\mathbf{D}_S$ 
may be different from that of $\mathbf{D}_0$, even then our 
computational framework is still valid and works as shown in the
representative problems outline in subsections plate with a hole 
\ref{SubSec:Plate_hole} and beam with three holes 
\ref{SubSec:Beam_three_holes}, where in $\mathbf{D}_T$ and 
$\mathbf{D}_S$ are chosen as follows:
%
\begin{subequations}
 \label{Eqn:General_DT_DS}
  \begin{align}
  %%
  \mathbf{D}_T &= 
  \left(\begin{array}{cc}
  \cos(\theta) & -\sin(\theta) \\ 
  \sin(\theta) & \cos(\theta)
  \end{array}\right)
  %
  \left(\begin{array}{cc}
  d_{1}^T & 0 \\ 
  0 & d_{2}^T
  \end{array}\right)
  %
  \left(\begin{array}{cc}
  \cos(\theta) & \sin(\theta) \\ 
  -\sin(\theta) & \cos(\theta)
  \end{array}\right) \\
  %%
  \mathbf{D}_S &= 
  \left(\begin{array}{cc}
  \cos(\theta) & -\sin(\theta) \\ 
  \sin(\theta) & \cos(\theta)
  \end{array}\right)
  %
  \left(\begin{array}{cc}
  d_{1}^S & 0 \\ 
  0 & d_{2}^S
  \end{array}\right)
  %
  \left(\begin{array}{cc}
  \cos(\theta) & \sin(\theta) \\ 
  -\sin(\theta) & \cos(\theta)
  \end{array}\right)
  %%
  \end{align}
\end{subequations}
%
%\end{remark}

%=============================================;
%  Subsection: Numerical h-convergence study  ;
%=============================================;
\subsection{Numerical $h$-convergence study}
\label{Sec:Convergence Study}
In this subsection, we perform a numerical $h$-convergence study 
by employing the proposed computational framework on a coupled 
deformation-diffusion problem. Herein, by $h$-convergence we 
mean the overall convergence of the proposed framework with 
respect to the refinement of the computational mesh (but still 
maintaining the same order of interpolation within each finite 
element). Since the non-negative solver for diffusion works only 
for low-order finite element, we employ low-order finite elements 
in all our numerical simulations. 
%
\emph{It should be noted that for each successful coupled analysis 
  using the proposed computational framework, the staggered 
  coupling algorithm should converge. For each iteration in 
  the staggered coupling algorithm, the active-set strategy 
  in the non-negative solver for the diffusion problem should 
  converge.}

We employ the method of manufactured solutions \cite{Knupp_Salari_2003} 
in this convergence study. The computational domain is taken as 
a bi-unit square ($0 \leq x \leq 1$ and $0 \leq y \leq 1$). The 
displacement vector is given by 
%--------------------------;
%  Equation: Displacement  ;
%--------------------------;
\begin{subequations}
  \label{Eqn:displacement_convergence_study}
  \begin{align}
    u(x,y) &= \frac{1}{\pi} \sin(\frac{\pi x}{2}) 
    \sin(\frac{\pi y}{2}) \\
    % 
    v(x,y) &= \frac{1}{\pi} \cos(\frac{\pi x}{2}) 
    \cos(\frac{\pi y}{2})
  \end{align}
\end{subequations}
% 
The concentration is given by 
%---------------------------;
%  Equation: Concentration  ;
%---------------------------;
\begin{align}
  \label{Eqn:concentration_convergence_study}
  c(x,y) = 1 + \frac{1}{\pi} \sin(\frac{\pi x}{2}) 
  \sin(\frac{\pi y}{2})
\end{align}
%
Note that the concentration given in the above equation is 
non-negative in the whole computational domain. The following 
parameters are assumed in the convergence study: 
%------------------------------------;
%  Equation: Convergence parameters  ;
%------------------------------------;
\begin{align}
  &\mu_0 = \pi + 2, \; \mu_1 = -\pi, \; \lambda_0 = 2, \; 
  \lambda_1 = -1, \; \rho = 1, \; E_{\mathrm{ref}} = 0.0001,  
  \nonumber \\
  % 
  &c_{\mathrm{ref}} = 1, \; \eta_T = 1, \; \eta_S = 1, \;
  \beta_T = 2, \; \beta_S = 2, \; \gamma_S = \frac{\beta_S - 1}
  {\exp[\eta_S E_{\mathrm{ref}}] - 1}, \nonumber \\
  % 
  &\mathbf{D}_0 = 2 \; \mathbf{I}, \; \mathbf{D}_T = \beta_T 
  \mathbf{D}_0, \; \mathbf{D}_S = \beta_S \mathbf{D}_0
  % 
\end{align}
%
The volumetric source for the diffusion problem is given by
%-------------------------------;
%  Equation: Volumetric source  ;
%-------------------------------;
\begin{align}
  \label{Eqn:Coupled_volumetric_source_convergence}
  f(x,y) &= \pi \sin(\frac{\pi x}{2}) \sin(\frac{\pi y}{2}) 
  \left(\left(1 - \gamma_S \right) + \gamma_S \; \mathrm{exp} 
    \left[\cos(\frac{\pi x}{2})\sin(\frac{\pi y}{2}) \right] 
  \right) \nonumber \\
  % 
  &- \frac{\pi \gamma_S}{4} \sin(\pi x) \cos(\pi y) \mathrm{exp}
  \left[\cos(\frac{\pi x}{2}) \sin(\frac{\pi y}{2}) \right]
\end{align}  
% 
The specific body force for the deformation problem is given by 
%---------------------------------;
%  Equation: Specific body force  ;
%---------------------------------;
\begin{align}
  \label{Eqn:Coupled_body_force_convergence}
  \mathbf{b}(x,y) = \left(\begin{array}{c}
      \pi \sin(\frac{\pi x}{2}) \sin(\frac{\pi y}{2}) + 
      \frac{\pi}{4} \cos(\pi x) (1 - \cos(\pi y))  \\ 
      %
      \pi \cos(\frac{\pi x}{2}) \cos(\frac{\pi y}{2}) - 
      \frac{\pi}{4} \sin(\pi x) \sin(\pi y)
    \end{array}\right)
\end{align}
%
The boundary value problem is pictorially described in Figure 
\ref{Fig:Coupled_convergence_pictorial}. The tolerance in the 
stopping criterion for the staggered coupling algorithm is 
taken as $\epsilon^{(c)}_{\mathrm{TOL}} = 10^{-8}$. 
%
A hierarchy of meshes similar to the ones shown in Figure 
\ref{Fig:Coupled_convergence_mesh} is employed in the numerical 
convergence study. 
%
In Figure \ref{Fig:Coupled_convergence_conc_comparison}, the 
obtained numerical solution using the mesh shown in Figure 
\ref{Fig:Coupled_convergence_T3_mesh} is compared with the 
analytical solution. The convergence of the proposed coupled 
framework is illustrated in Figures \ref{Fig:Coupled_convergence_conc} 
and \ref{Fig:Coupled_convergence_disp} for three-node triangular and 
four-node quadrilateral elements with respect to $L^{2}$-norm and 
$H^{1}$-seminorm, and the proposed computational framework performed 
well. 

In the subsequent subsections, we employ the proposed computational 
framework to solve various finite domain practical problems. Using these 
we illustrate how the tension, compression and shear in the solid affect 
the (steady-state) diffusion process, and how the concentration of the 
diffusant affect the deformation of the solid. 
%
The values of the parameters that are common to all the test problems 
are presented in Table \ref{Table:Coupled_common_parameters}. We have 
given the values for the volumetric source and body force for all the 
test problems in Table \ref{Table:Coupled_fx_bx}. 

%--------------------------------------;
%  Table: Values of common parameters  ;
%--------------------------------------;
\begin{table}
  \caption{Values of the parameters that are the same in all test 
    problems (except for the one in the numerical $h$-convergence). 
    \label{Table:Coupled_common_parameters}}
  \begin{tabular}{cc} \hline
    Parameter & value \\ \hline
    $\rho$ & 1 \\
    $c_{\mathrm{ref}}$ & 1 \\     
    $E_{\mathrm{ref}}$ & 0.0001 \\
    $\lambda_0$ & $+10^{6}$ \\
    $\mu_0$ & $+10^{6}$ \\
    $\lambda_1$ & $-9 \times 10^{5}$ \\
    $\mu_1$ & $-9 \times 10^{5}$ \\ \hline
  \end{tabular}
\end{table}
%-------------------------------------------;
%  Table: Volumetric source and body force  ;
%-------------------------------------------;
\begin{table}
  \caption{Volumetric source $f(\mathbf{x})$ and body force 
    $\mathbf{b}(\mathbf{x})$ for various test problems. 
    \label{Table:Coupled_fx_bx}}
  \begin{tabular}{lcc} \hline
    Test problem & $f(\mathbf{x})$ & $\mathbf{b}(\mathbf{x})$ \\ \hline
    Cantilever beam with edge shear & 10000 & $\mathbf{0}$ \\ 
    Simply supported beam under self-weight & 1000 & $-10 \; \hat{\mathbf{e}}_y$ \\
    Fixed beam under self-weight & 100 & $-10 \; \hat{\mathbf{e}}_y$ \\
    Plate with a hole under self-weight & 0 & $-10 \; \hat{\mathbf{e}}_y$ \\
    Beam with three holes under self-weight & 0 & $-10 \; \hat{\mathbf{e}}_y$ \\ \hline
  \end{tabular}
\end{table}


==> Sections/S4_P2.tex <==
%===============================================;
%  Subsection: Cantilever beam with edge shear  ;
%===============================================;
\subsection{Cantilever beam with edge shear}
\label{SubSec:Cantilever_beam_edge_shear}
The purpose of this test problem is to illustrate the affect of 
$\mathbf{D}_S$ on the coupled response. We consider a cantilever 
beam with a uniform edge shear of $500$. The length of the beam 
is $1.0$, and the height of the beam is $0.1$. For the deformation 
problem, top and bottom surfaces are subjected to zero traction. 
For the diffusion problem, zero concentration is prescribed on 
the top and bottom surfaces, and zero flux is prescribed on the 
left and right surfaces. The boundary value problem is pictorially 
described in Figure \ref{Fig:Coupled_CB_edgeshear}.

We have employed a structured mesh using four-node quadrilateral 
elements with 21 nodes along each side of the domain (see the mesh 
in Figure \ref{Fig:Diffusion_CB_Edgeshear}). The stopping criterion 
is again taken as $\epsilon^{(c)}_{\mathrm{TOL}} = 10^{-8}$. We have 
considered three different values for $\Phi_S$: 5, 10, and 20. The 
other parameters used in the coupled analysis are as follows:
%-----------------------------------------------------------;
%  Equation: Parameters in cantilever beam with edge shear  ;
%-----------------------------------------------------------;
\begin{align}
  \theta = \frac{\pi}{6}, \; d_1 = 1, \; d_2 = 1, \; 
  \Phi_T = 2, \; \eta_T = 100, \;  \eta_S = 1    
\end{align}
%
The contour profiles for the concentration for these three values are shown 
in Figure \ref{Fig:Diffusion_CB_Edgeshear}. As expected, the diffusant 
accumulated near the right side of the domain (where the uniform edge 
shear is applied). In Table \ref{Tab:CB_EdgeShear}, we have presented 
the maximum concentration and the number of iterations taken by the 
staggered coupling algorithm for the chosen values of $\Phi_S$. One 
can observe that as $\Phi_S$ increases, the staggered coupling algorithm 
takes fewer iterations. This can be explained as $\Phi_S$ increases, the 
diffusivity increases and the diffusant is more uniformly distributed (which 
is evident from Figure \ref{Fig:Diffusion_CB_Edgeshear}).

%------------------------------------------;
%  Table: Cantilever beam with edge shear  ; 
%------------------------------------------;
\begin{table}
  \centering
  \caption{Cantilever beam with edge shear: The table presents the maximum 
  concentration and the number of iterations taken by the staggered coupling 
  algorithm for various values of $\Phi_S$. (Note that the minimum concentration 
  in all the cases is zero.) \label{Tab:CB_EdgeShear}}
  \begin{tabular}{ccc}
    \hline
    $\Phi_S$ & Max. concentration & Iterations \\
    \hline
    $5$ & $4.257 \times 10^{-1}$ & $14$ \\
    $10$ & $2.187 \times 10^{-1}$ & $9$ \\
    $20$ & $1.107 \times 10^{-1}$ & $7$ \\
    \hline
  \end{tabular}
\end{table}

%=======================================================;
%  Subsection: Simply supported beam under self weight  ;
%=======================================================;
\subsection{Simply supported beam under self-weight}
\label{SubSec:Simply_supported_beam}
The purpose of this test problem is to study the affect of $\eta_S$ 
on the coupled response, and to illustrate the competitive effects 
of shear and tension/compression on the diffusion process. We consider 
a simply supported beam under self-weight with traction-free surfaces. 
The boundary value problem is pictorially described in Figure 
\ref{Fig:Coupled_SS_selfweight}.

The tolerance for the stopping criterion in the staggered coupling 
algorithm is taken as $\epsilon^{(c)}_{\mathrm{TOL}} = 10^{-5}$. 
We have employed a structured mesh using four-node quadrilateral 
element with 21 nodes along each side of the domain (see the mesh 
in Figure \ref{Fig:Diffusion_SS_selfweight}). We have considered three 
values for $\eta_S$: $1$, $10^3$  and $2 \times 10^4$. The other 
parameters used in this test problem are as follows:
%-------------------------------------------------------------------;
%  Equation: Parameters in simply supported beam under self-weight  ;
%-------------------------------------------------------------------;
\begin{align}
  \theta = \frac{\pi}{6}, \; d_1 = 1, \; d_2 = 1, \; 
  \Phi_T = 10, \; \Phi_S = 10, \;\eta_T = 1 
\end{align}

%--------------------------------------------------;
%  Table: simply supported beam under self-weight  ; 
%--------------------------------------------------;
\begin{table}
  \centering
  \caption{Simply supported beam under self-weight: The table presents 
  the maximum concentration and the iterations taken by the staggered 
  coupling algorithm for various values of $\eta_S$. (Note that the 
  minimum concentration in all the cases is zero.)}
  \label{Tab:SS_selfweight}
  \begin{tabular}{ccc}
    \hline
    $\eta_S$ & Max. concentration & Iterations \\
    \hline
    $1$ & $7.205 \times 10^{-1}$ & $10$ \\
    $10^3$ & $7.309 \times 10^{-1}$ & $10$ \\
    $2 \times 10^4$ & $9.365 \times 10^{-1}$ & $12$ \\
    \hline
  \end{tabular}
\end{table}

From Table \ref{Tab:SS_selfweight} one can infer that as $\eta_S$ 
increases the maximum concentration and iterations taken for 
convergence of staggered coupling algorithm increase. This is 
because for lower values of $\eta_S$ shear affects the diffusivity 
tensor more than the tension/compression and for higher values of 
$\eta_S$ tension/compression dominates. This is also evident in the 
numerical results presented in Figure \ref{Fig:Diffusion_SS_selfweight}. 
For lower values of $\eta_S$, the diffusant accumulated near the 
supports of the beam (where the shear is maximum). For higher values 
of $\eta_S$, the diffusant spreads deep into beam. An important 
feature to be noted is that the concentration profile curves up. 
This is because the diffusivity is higher in tension than in compression. 
This is physically meaningful, as, in general, the sizes of pores in the 
solid enlarge due to tension, shrink due to compression, and distort due 
to shear. The deformation-dependent diffusivity tensor $\mathbf{D}_
{\mathbf{E}_l}(\mathbf{x})$ given by equation \eqref{Eqn:Coupled_diffusivity} 
takes these factors into account. The next test problem highlights 
other important features of the proposed mathematical model. 

%============================================;
%  Subsection: Fixed beam under self weight  ;
%============================================;
\subsection{Fixed beam under self-weight}
\label{SubSec:Fixed_beam}
The purpose of this test problem is to study the affect of $\Phi_T$ 
on the coupled response and show that our model can capture the 
qualitative aspects of the experiments done by McAfee 
\cite{McAfee_JoCP_1958_v28_p218,McAfee_JoCP_1958_v28_p226}. 
A fixed beam of length unity and depth $0.1$ is subjected to self-weight. 
The top and bottom surfaces are traction-free. For the diffusion problem, 
the top and bottom surfaces have zero concentration, and the left and right 
surfaces have zero flux. The boundary value problem is pictorially 
described in Figure \ref{Fig:Coupled_FB_selfweight}.

The tolerance for the stopping criterion in the staggered coupling 
algorithm is taken as $\epsilon^{(c)}_{\mathrm{TOL}} = 10^{-7}$. We have 
employed a structured mesh using four-node quadrilateral element with 
21 nodes along each side of the domain (see the mesh in Figure 
\ref{Fig:Diffusion_FB_selfweight_mudunuru}). We have considered 
three different values for $\Phi_T$: 1, 5 and 7. The other parameters 
used in this test problem are as follows: 
%----------------------------------------------------------------;
%  Equation: Parameters assumed for fixed beam under self-weight  ;
%----------------------------------------------------------------;
\begin{align}
  \theta = 0, \; d_1 = 1, \; d_2 = 1, \; \Phi_S = 1, \; 
  \eta_T = 100, \; \eta_S = 1 
\end{align}

%---------------------------------------;
%  Table: Fixed beam under self-weight  ; 
%---------------------------------------;
\begin{table}
  \centering
   \caption{Fixed beam under self-weight: The table presents the maximum 
   concentration and the iterations taken by the staggered coupling algorithm 
   for various values of $\eta_T$. (Note that the minimum concentration in all 
   the cases is zero.)}
  \label{Tab:FB_selfweight}
  \begin{tabular}{ccc}
    \hline
    $\Phi_T$ & Max. concentration & Iterations \\
    \hline
    $1$ & $1.250 \times 10^{-1}$ & $2$ \\
    $5$ & $1.348 \times 10^{-1}$ & $5$ \\
    $7$ & $1.575 \times 10^{-1}$ & $8$ \\
    \hline
  \end{tabular}
\end{table}

In Table \ref{Tab:FB_selfweight}, we have presented the maximum 
concentration and number of iterations taken by the staggered 
coupling algorithm for chosen values of $\Phi_T$. One can observe 
that as $\Phi_T$ increases the maximum concentration and iterations 
taken increase. This results in the deformation-dependent diffusivity 
$\mathbf{D}_{\mathbf{E}_l}$ being 
high in tensile and low in compressive and shear regions of the beam. 
The diffusant accumulates in low diffusive areas such as the supports 
which are under shear and top section of the beam which is in compression. 
From Figure \ref{Fig:Diffusion_FB_selfweight_mudunuru} one can observe 
that the concentration profile which is initially around the central 
line of the beam curves up (the region of interest being around 0.12). 
This test problem shows the success of our 
mathematical model in predicting the underlying physical phenomena 
observed from the stress-induced experiments done by McAfee 
\cite{McAfee_JoCP_1958_v28_p218,McAfee_JoCP_1958_v28_p226}. 
The invariants which represent dilation and distortion in our model 
were instrumental in capturing the change in diffusivity under tension, 
compression and shear. Hence concentration curves towards the compression 
zone.

This type of curving of the concentration profile is not observed when 
one uses the model in which $\mathbf{D}_{\mathbf{E}_l} (\mathbf{x})$ 
depends only on $\|\mathbf{E}_l\|$. As mentioned in the Remark 
\ref{Remark:Coupled_norm_of_epsilon}, a diffusivity model based on 
the frobenius norm of $\mathbf{E}_l$ cannot capture the change in 
diffusivity tensor under tension, compression and shear deformations. 
The diffusivity tensor as per Reference 
\cite{Karra_Rajagopal_degradation_arXiv_2010} and the parameters assumed 
for the numerical study are given by:
%------------------------------------------;
%  Equation: Diffusivity (Norm of epsilon) ;
%------------------------------------------;
\begin{subequations}
  \label{Eqn:Coupled_diffusivity_norm}
  \begin{align}
      &\mathbf{D}_{\mathbf{E}_l} (\mathbf{x})  = \mathbf{D}_{0}(\mathbf{x}) + 
      \left(\mathbf{D}_{\infty}(\mathbf{x}) - \mathbf{D}_{0}(\mathbf{x}) \right) 
      \left(1 \; - \; \exp[-\lambda \|\mathbf{E}_l\|] \right) \\
      %
      &\theta = 0, \; d_1 = 1, \; d_2 = 1, \; \lambda = 100, \; 
       \mathbf{D}_{\infty} = 10 \, \mathbf{D}_{0}
  \end{align}
\end{subequations}
%
The concentration profile as illustrated in Figure 
\ref{Fig:Diffusion_FB_selfweight_karra} is always around 
the central line and does not curve up for any value of 
$\mathbf{D}_{\infty}$ and $\lambda$.


==> Sections/S4_P3.tex <==
%============================================;
%  Subsection: Rectangular domain with holes ;
%============================================;
\subsection{Degradation/healing of rectangular domains with holes}
\label{SubSec:Rectangular_domain_with_holes}
In the following subsections, we highlight the importance of non-negative 
solutions and its impact on coupled deformation-diffusion analyses of 
rectangular domains with holes. We compare the non-negative formulation 
with the standard Galerkin formulation using two representative problems. 
We shall model $\mathbf{D}_T$ and $\mathbf{D}_S$ by the equations 
\eqref{Eqn:General_DT_DS} in which $d_{j}^i$ is different from $d_{j}$ 
where $i \, = T, \, S$ and $j \, = 1, \, 2$. In both numerical studies here, 
the tolerance for the stopping criterion in the staggered coupling algorithm 
is taken as $\epsilon^{(c)}_{\mathrm{TOL}} = 10^{-5}$ and three-node 
triangular unstructured meshes were used (see Figures 
\ref{Fig:Plate_with_hole_pictorial} and 
\ref{Fig:Beam_with_three_holes_concentration}).

%===================================================;
%  Subsection: Plate with a hole under self-weight  ;
%===================================================;
\subsubsection{Plate with a hole under self-weight}
\label{SubSec:Plate_hole}
The purpose of this test problem is to study the importance 
of non-negative constraint in coupled-deformation-diffusion analyses.
Herein, we perform coupled analysis for a square plate with a square 
hole under self-weight. The computational domain $\Omega$ is the region 
in-between a bi-unit square plate and a square hole of length $\frac{1}{9}$. 
The boundary conditions for displacements at the hole and traction for the 
plate are equal to zero. The concentration at the hole is maintained at $1$ 
while that at boundary of the plate is equal to $0$. The boundary value 
problem is pictorially described in Figure  \ref{Fig:Plate_with_hole_pictorial}. 
The other parameters assumed in the analysis of the coupled problem are as follows:
%------------------------------------------------------;
%  Equation: Parameters assumed for plate with a hole  ;
%------------------------------------------------------;
\begin{align}
\label{Eqn:Plate_with_hole_parameters}
    &\theta = \frac{\pi}{3}, \; \eta_T = 1, \; 
    \eta_S = 1, \; d_1 = 10000, \; d_1^T = 11000, \;
    d_1^S = 11000, \; d_2 = 1, \; d_2^T = 10, \; d_2^S = 5 
\end{align}
%
From Figure \ref{Fig:Plate_with_hole_concentration} it is evident that the proposed 
non-negative formulation satisfies the above condition and produces physically 
meaningful concentration while the standard Galerkin formulation predicts otherwise. 
The comparison of the concentration and degradation profiles for the standard Galerkin 
vs. the non-negative formulation given in Figures \ref{Fig:Plate_with_hole_concentration} 
and \ref{Fig:Plate_with_hole_degradation} shows that the Galerkin formulation violates 
the non-negative constraint. The obtained negative values for the concentration are not 
just numerical noise (see Table \ref{Tab:Plate_with_hole_tabular}).
%----------------------------;
%  Table: Plate with a hole  ; 
%----------------------------;
\begin{table}
  \centering
  \caption{Plate with a hole under self-weight: The table presents the 
  minimum concentration, degradation index and the iterations taken 
  by staggered coupling algorithm using the standard single-field formulation. 
  Analysis is done for various values of $\left(d_1,d_1^T,d_1^S \right)$ by 
  keeping other parameters in equations \ref{Eqn:Plate_with_hole_parameters} 
  fixed.} \label{Tab:Plate_with_hole_tabular}
	\begin{tabular}{ccccc}
	  \hline
	  $\left(d_1,d_1^T,d_1^S\right)$ & 
	  Min. concentration & Degradation Index & Iterations   & Iterations  \\
	  %%%
	  $\,$ & $\,$ & (\% of nodes violated) & (Galerkin) &
	  (non-negative) \\
	  \hline
	  $(1,10,10)$ & 0 & 0 & 9 & 9  \\
	  $(10,30,20)$ & 0 & 0 & 8 & 8  \\
	  $(100,120,110)$ & $-3.301 \times 10^{-3}$  & 25.15 & 6 & 21  \\
	  $(1000,1200,1100)$ & $-3.586 \times 10^{-2}$ & 32.76 & 5 & 22  \\
	  $(10000,11000,11000)$ & $-4.398 \times 10^{-2}$ & 34.07 & 4 & 8  \\
	  \hline
	\end{tabular}
\end{table}

%=====================================;
%  Subsection: Beam with three holes  ;
%=====================================;
\subsubsection{Beam with three holes under self-weight}
\label{SubSec:Beam_three_holes}
The purpose of this test problem is to show that as number 
of holes increase, the spatial extent and magnitude of violation 
of the non-negative constraint by the Galerkin formulation increase 
dramatically. Herein, we perform coupled deformation-diffusion 
analysis for a beam with three square holes under self-weight. 
The computational domain $\Omega$ is the region in-between a 
beam of length $10.0$ and height $1.0$ and three square holes 
each of length $0.4$. The boundary conditions for displacements 
at the holes and traction for the beam are equal to zero. The 
concentration at the holes is maintained at $1$ while that at boundary 
of the beam is equal to $0$. The boundary value problem is pictorially 
described in Figure \ref{Fig:Beam_with_three_holes_pictorial}. The other 
parameters assumed in the analysis of the coupled problem are as follows:
%---------------------------------------------------------;
%  Equation: Parameters assumed for beam with three holes  ;
%---------------------------------------------------------;
\begin{align}
  \label{Eqn:Beam_with_three_hole_parameters}
    &\theta = \frac{\pi}{4}, \; \eta_T = 1, \; \eta_S = 1, \; 
    d_1 = 10000, \; d_1^T = 20000, \; d_1^S = 15000, \; d_2 = 1, \; 
    d_2^T = 5, \; d_2^S = 2 
\end{align}
%
From Figures \ref{Fig:Beam_with_three_holes_concentration} 
and \ref{Fig:Beam_with_three_holes_degradation} it is evident that as 
the number of holes increase, the regions of negative concentration 
obtained from the standard Galerkin formulation also increases. 
Also from Tables \ref{Tab:Plate_with_hole_tabular} and 
\ref{Tab:Beam_with_three_hole_tabular} it is evident that the 
negative concentration obtained from numerical study on beam with 
three holes is $1.35$ times that of the plate with a hole. 

%--------------------------------;
%  Table: Beam with three holes  ; 
%--------------------------------;
\begin{table}
  \centering
	\caption{Beam with three holes under self-weight: The table presents 
	the minimum concentration, degradation index and the iterations taken 
	by staggered coupling algorithm using the standard single-field formulation. 
	Analysis is done for various values of $\left(d_1,d_1^T,d_1^S \right)$ 
	by keeping other parameters in equations 
	  \ref{Eqn:Beam_with_three_hole_parameters} fixed.}
	\label{Tab:Beam_with_three_hole_tabular}
	\begin{tabular}{ccccc}
	  \hline
	  $\left(d_1,d_1^T,d_1^S\right)$ & 
	  Min. concentration & Degradation Index & Iterations   & Iterations  \\
	  %%%
	  $\,$ & $\,$ & (\% of nodes violated) & (Galerkin) &
	  (non-negative) \\
	  \hline
	  $(1,10,10)$ & 0 & 0 & 8 & 8  \\
	  $(10,50,30)$ & 0 & 0 & 8 & 8  \\
	  $(100,200,150)$ & $-3.150 \times 10^{-2}$  & 30.69 & 6 & 8  \\
	  $(1000,2000,1500)$ & $-5.665 \times 10^{-2}$ & 31.14 & 6 & 6  \\
	  $(10000,20000,15000)$ & $-5.948 \times 10^{-2}$ & 31.14 & 6 & 16  \\
	  \hline
	\end{tabular}
\end{table}

%\begin{remark}
%  \label{Rem:Negative_Concentration_Machine_Precesion}
%  The maximum value of the negative concentration obtained as per Tables 
%  \ref{Tab:Plate_with_hole_tabular} and \ref{Tab:Beam_with_three_hole_tabular} 
%  is less than the machine precision. The machine precision on a 64-bit 
%  machine is equal to $-2.2204 \times 10^{-16}$. This is of considerable 
%  importance since one can get negative value of concentration due to the 
%  round-off errors from the 
%  machine. Thus the negative concentrations obtained from the standard Galerkin 
%  formulation includes the values which are less than and equal to machine 
%  epsilon. The values of concentration profiles and the regions in which 
%  concentration is less than the machine precision are shown in Figures 
%  \ref{Fig:Plate_with_hole_degradation} and \ref{Fig:Beam_with_three_holes_degradation}. 
%  One can see a clear difference from Figure \ref{Fig:Plate_with_hole_concentration} to 
%  Figure \ref{Fig:Plate_with_hole_degradation} and Figure 
%  \ref{Fig:Beam_with_three_holes_concentration} to Figure 
%  \ref{Fig:Beam_with_three_holes_degradation} when one excludes 
%  the concentration values above the machine epsilon.
%\end{remark}

From Tables \ref{Tab:Plate_with_hole_tabular} and 
\ref{Tab:Beam_with_three_hole_tabular}, one can see that as the directional 
diffusivities $d_1$, $d_1^T$ and $d_1^S$ increase the minimum concentration 
(which is initially zero) becomes negative under the Galerkin formulation. This 
negative value of concentration and the degradation index (which represents 
the \% of nodes at which concentration is negative) increases as these diffusivities 
increase. The proposed non-negative formulation does not give negative values for 
the concentration for any values for these how these diffusivities. 
%
This is quite important because the material properties of the 
solid are dependent on the concentration obtained. From Figures 
\ref{Fig:Plate_with_hole_degradation} and \ref{Fig:Beam_with_three_holes_degradation}, 
one can observe that the standard Galerkin method predicts that some regions 
are \textit{healing} due to the \textit{negative} values of the concentration 
which is physically unrealistic. The non-negative solver employed always gives 
non-negative concentration and shows that material is \textit{degrading 
  everywhere}.

%===================================================;
%  Subsection: Performance of the staggered scheme  ;
%===================================================;
\subsection{Performance of the staggered scheme and the active-set strategy}
The convergence histories of the staggered coupling algorithm 
for the aforementioned test problems are shown in Figure 
\ref{Fig:Coupled_staggered_conc}. Note that the convergence 
of the staggered coupling algorithm is monotonic for the test 
problems on degradation/healing of beams. But the convergence 
is not monotonic for the test problem on degradation/healing 
of rectangular domain with holes, which is illustrated in Figure 
\ref{Fig:Coupled_staggered_conc_domain_holes}). 
%
Figure \ref{Fig:Coupled_active_set_conc} shows the number of 
active-strategy iterations required for solving the constrained 
optimization problem for each iteration in the staggered coupling 
algorithm. 


==> Sections/S5_Coupled_Conclusions.tex <==
%*****************************************;
%                                         ;
%  Section: S7_Coupled_Conclusions.tex    ;
%                                         ;
%*****************************************;
\section{CONCLUSIONS}
\label{Sec:Coupled_Conclusions}
Many technologically and biologically important processes 
are coupled deformation-diffusion problems. Lately, there 
is a surge in research activity in studying coupled 
deformation-diffusion problems. However, in all these research 
efforts it has not been recognized that many popular numerical 
formulations and existing computational packages predict unphysical 
negative solutions for the concentration of the diffusant, and this 
is more prominent in the case of a medium which has high directional 
diffusivities. Concentration of a chemical is a non-negative quantity, 
and this property has to be preserved to obtain physically meaningful 
numerical solution for a coupled deformation-diffusion problem. 

We proposed a mathematical model for coupled deformation-diffusion 
analysis, which is suitable to model degradation/healing of materials 
and structures. The model is \emph{fully} coupled in the sense that the 
deformation process is affected by the diffusion process, and the diffusion 
process is in turn affected by the deformation of solid. One of the main 
contributions is that we have presented a robust computational framework 
for solving coupled deformation-diffusion problems. The computational 
framework includes a non-negative formulation for (tensorial) diffusion 
equation, a numerical solver for the deformation of the solid, and a 
staggered coupling algorithm. An important aspect of the computational 
framework is that it always produces physically meaningful non-negative 
values for the concentration of the diffusant on any computational grid 
(with low-order finite elements) even for a medium which has high directional 
diffusivities. We have illustrated the robustness of the computational framework 
on representative numerical examples. We have studied systematically the 
affect of the deformation on the diffusion process on various practically 
important problems.

